Nonuniqueness and structural stability of self-consistent models of elliptical galaxies

(Abridged:) Schwarzschild's method was used to construct equilibrium solutions to the collisionless Boltzmann equation corresponding to a Plummer sphere, which were compared with analytical results to test the robustness of the numerical method and its efficiency in probing the degeneracy of the solution space. The method was then used to construct triaxial equilibria with no known analytical solutions and to study their nonuniqueness. The model that was studied, the triaxial Dehnen potential, contains a central density cusp and admits both regular and chaotic orbits. It was found that, for a weak density cusp, self-consistent models do not exist if the chaotic orbits are assumed to be completely mixed so as to yield a time-independent building-block: only the innermost 65% of the mass can be mixed. In these inner regions, it is possible to obtain alternative solutions that contain significantly different numbers of chaotic orbits, yet yield (at least approximately) the same mass density distribution. However, it is not clear whether these solutions are truly time-independent, since the unmixed chaotic orbits in the outer regions, which do not sample an invariant measure, can cause secular evolution. When using Schwarzschild's method, one must be very careful to sample accessible phase space as comprehensively and as densely as possible, while ensuring that each orbit is a truly time-independent building block. Some of the numerical equilibria were sampled to generate initial conditions for N-body simulations to test the structural stability of the models. Preliminary work showed that no catastrophic evolution takes place, but there is a weak tendency for the configuration to become more nearly axisymmetric over several dynamical times. It is not yet clear whether this tendency is real or a numerical artifact.

==> Aux/BioPage.tex <==
\vspace*{65pt}
\centerline{BIOGRAPHICAL SKETCH}
\vspace{.5in}

%%%% The Bio goes here.
\DoubleSpace

\input{\Misc/Bio}

\SingleSpace


==> Aux/Signatures.tex <==
\thispagestyle{empty}
\SingleSpace

\newcommand{\CertPar}[2]{ 
\vbox{I certify that I have read this study and that 
in my opinion it conforms to acceptable standards of scholarly presentation 
and is fully adequate, in scope and quality, as a 
\lowercase\expandafter{\ThesisType}for the degree of 
\DegreeType\hspace{-1.0ex}.

\vspace*{.25in}
\noindent\hspace*{3in}\hrulefill \\
\hspace*{3in}#1 \\
\hspace*{3in}#2

\vspace*{.25in}
}
}

\openin\InStream=\Info/Committee

\read\InStream to \CName  % advisor's name
\read\InStream to \CDept  % advisor's dept
\CertPar{\Advisor, Chairman}{\CDept}

\Done=0
\LOOP\ifnum\Done=0
   \ifeof\InStream\global\Done=1
   \else
     \read\InStream to \CName
     \ifeof\InStream{}\else
        \read\InStream to \CDept
        \ifeof\InStream{}\else
           \CertPar{\CName}{\CDept}\fi\fi
   \fi
\REPEAT
\closein\InStream

This \lowercase\expandafter{\ThesisType}was submitted to the Graduate 
Faculty of the Department of \Department in the College of Liberal Arts 
and Sciences and to the Graduate School and was accepted as partial 
fulfillment of the requirements for the degree of {\DegreeType}\hspace{-1.0ex}.

\vspace*{0.25in}
\noindent\makebox[3in][l]{\GradMonth\ \GradYear}\hrulefill \\
\hspace*{3in}Dean, Graduate School


==> Chapters/Definitions.tex <==
% \input{\Chapters/Definitions/Theorem}	% thm environments
\input{\Chapters/Definitions/Misc}
% \input{\Chapters/Definitions/GeneralMath}
% \input{\Chapters/Definitions/Thesis}	% specific to *my* thesis


==> Chapters/Definitions/Misc.tex <==
\newcommand{\Figure}[4]{
\begin{figure}
\epsfxsize=#2
\centerline{\leavevmode\epsfbox{#1}}
\caption{#3}
\FigLabel{#4}
\end{figure}}

%%%%%%%%   A little macro to make notes starting in margin.
%        I find it useful to remind myself what I still need to do in
%        a particular section. The variable ShowNotes is used to 
%        display, or hide all NOTEs. It's defined at the top of Thesis.tex.
%
\newcommand{\NOTE}[1]{
\ifx\ShowNotes\True
\vbox{\vspace*{0.25in}\hrule
\vspace*{0.15in}#1
\vspace*{0.15in}\hrule}\marginpar{NOTE}
\vspace{0.25in}
\fi}
%
%%%%%%%%


%%%%%%%%   Makes a list with each item labelled with a bullet
%
\newenvironment{Bullets}{\begin{list}{$\bullet$}{}}{\end{list}}
%
%%%%%%%%



==> Chapters/conclusions.tex <==
\chapter{CONCLUSIONS}

This dissertation had two main goals. The first was to understand some of
the subtleties involved in applying Schwarzschild's method for the
construction of numerical solutions (distribution functions) of the
collisionless Boltzmann equation. This was effected by applying the method
to a simplified problem, namely the construction of a self-consistent
Plummer sphere, for which analytical solutions are known and can be used
to judge the quality of the numerical solutions obtained via
Schwarzschild's method. Of particular interest was an investigation of the
ability of the numerical method to reproduce at least some of the
degeneracy of the solutions that is known to be there from analytical
work.

The second aim was to use the expertise gained from the test problem to
construct a numerical distribution function of a triaxial galaxy with a
central cusp, where chaos is expected to play an important role and no
known analytical solutions exist. The objectives here were (i) to compare
the results from this study with results reported by \citet{MerFri96} who
constructed models of the same potential but in a slightly different way,
and (ii) to explore the degeneracy of the solutions, in particular whether
it is possible to have two alternative distribution functions, both
corresponding to the same mass density distribution, but containing
significantly different numbers of chaotic orbits.

The principal moral derived from the extensive use of Schwarzschild's
method in this work is that the importance of a good library of orbital
templates cannot be overemphasized. The initial conditions have to be
selected carefully so as to provide as comprehensive a coverage of phase
space as possible. This usually means that one has to have a good
understanding of the orbital structure of the system to be modeled.
Failure to include enough orbits, or an injudicious choice of initial
conditions that would miss important families of orbits or violate the
symmetries of the system, could lead to unphysical results: one could end
up with a solution that does not really exist or miss solutions that do
exist. The fact that the inversion problem lying at the heart of
Schwarzschild's method is ill-conditioned only exacerbates the situation.

The principal physical conclusion is that it seems possible to achieve
self-consistency for the $\gamma=1$, weak-cusp triaxial Dehnen model, at
least in the innermost 13 shells, corresponding to the innermost 65\% of
the mass of the system. Furthermore, this could be done allowing for
substantial variations in the measure of strongly chaotic orbits. It is
not clear why self-consistency cannot be attained in the outer regions.
One obvious possibility is that the time-averaged distribution of the
outer chaotic orbits does not accurately sample the invariant measure. The
rate at which orbital ensembles approach the invariant measure can vary
substantially with energy and choice of potential. Similar sampling
problems with the Plummer sphere models may have been the cause of
observed irregularities in the tangential velocity distributions. However,
these irregularities may simply reflect the fact that only five values of
angular momentum were considered for each shell. This latter possibility
will be checked by repeating the above calculations allowing for more
values of angular momentum. Furthermore, pinning down the exact number of
chaotic orbits in the triaxial Dehnen model is not trivial because of
the difficulty in distinguishing between regular and confined chaotic
orbits. Neither \citet{MerFri96} nor this work claim to have completely
solved this problem.

One obvious step in this direction would be to repeat the integration of
all library orbits for considerably longer times, which would allow some
confined chaotic orbits to become unconfined, thus enabling one to better
distinguish between regular and chaotic orbits. Once the chaotic orbits of
the ensemble have been identified, they can be integrated for very long
times to yield a better approximation to the invariant measure. 

Being able to distinguish properly between regular and chaotic orbits is
crucial if one is to construct a truly self-consistent model. The true
invariant measure of chaotic orbits at any given energy will in general
contain both strongly chaotic contributions and much weaker contributions,
the latter corresponding to orbits confined near regular islands. It
follows that a proper ``mixing'' of the chaotic orbits necessarily
involves combining confined and strongly chaotic orbits with the proper
relative weight. Failure to do so means that one will likely construct an
approximation to a near-equilibrium, characterized by near-invariant
chaotic distributions, rather than to a true invariant distribution
\citep{Pfe86, HabKan97}.

\citet{MerFri96} present the argument that mixing the chaotic orbits in
the outer regions, where dynamical times are long, may not be required for
the system to be (nearly) time-independent over a Hubble time. However,
such an expectation may not be realistic, for at least three reasons.
First, the orbits in the library actually represent orbital {\em
templates} and their time independence has to be guaranteed irrespective
of the length of a Hubble time (see discussion on page
\pageref{2.pag.whynofixedt}). Second, small irregularities associated with
the graininess of the system (\eg due to close encounters) can
dramatically accelerate phase-space transport (\eg Arnold web penetration)
in less than a Hubble time \citep{Pfe86, HabKan97}. Third, galaxies had to
form and evolve to their present configurations. It may be unrealistic to
expect that during their more violent past, galaxies were able to keep
chaotic subdomains of their phase space unmixed. One might still argue
that {\em after} a galaxy settles to a more relaxed state, phase-space
diffusion could fill chaotic regions that are relatively isolated from
each other via the Arnold web. However, such an argument implies a slow
evolution with time that would alter the mass distribution and violate the
initial assumption of self-consistency.

Another important extension of this work involves considering other values
of $\gamma$, \eg $\gamma = 2$ and $\gamma \approx 0$. Such work would
provide insights into the question of whether the nonexistence of
self-consistent solutions really reflects the strength of the cusp. This
is not completely obvious, since self-consistency breaks at large radii,
where one might expect that the effects of the cusp would be especially
small. Conventional wisdom suggests that there should be no problem
constructing self-consistent models for the coreless case ($\gamma=0$),
but this has not been shown.

The other obvious question is whether these models are stable, so that
they can represent realistic configurations. This can and will be studied
by generating $N$-body realizations of the Schwarzschild models and
evolving them into the future. Work on this has already begun in
collaboration with E. Athanassoula of the Observatoire de Marseille using
their GRAPE-3 and GRAPE-4 facilities. GRAPE (GRAvity PipE) is a massively
parallel special-purpose computer for $N$-body simulations of
gravitational systems \citep{MakTai97}. The particular configuration in
Marseille can reach a sustained speed of about 28 GFLOPS and can currently
handle up to $\sim 10^6$ particles (this number is only limited by the
host computer's physical memory). The system uses a tree code, specially
adapted for GRAPE's architecture.

\begin{figure}[t]
\begin{center} 
\epsfig{file=Figures/fig4-1.eps,width=12cm}

\footnotesize{(a)}

\epsfig{file=Figures/fig4-2.eps,width=12cm}

\footnotesize{(b)}

\end{center} 

\caption{\label{4.fig.1} The $x-y$ and $x-z$ projections of an $N$-body
simulation of the $\gamma=1$ triaxial Dehnen potential. (a) Near $t=0$;
(b) after several inner-region dynamical times.}
\end{figure}


The triaxial Dehnen DFs were sampled in the following way: if the weight
$w_o$ of a particular orbit, normalized such that $\sum_{o=1}^{N_o} w_o =
1$, was greater than a random number in the interval [0,1], then an
$N$-body particle was generated, with the position and velocity of a
random point along that orbit's path, as sampled from the library of
orbital templates. This process was repeated until the intended number of
$N$-body particles was reached. In order to help reduce large-scale
fluctuations in the potential, induced by the random sampling process, the
initial conditions were only sampled in the positive octant, and seven
more symmetrical initial conditions were created in the remaining octants.
Such measures are crucial for stability studies \citep{SelAth86}.

A small number of trial $N$-body realizations of Schwarzschild equilibria
using $10^5$ particles have already been performed with the aim of
checking whether the $N$-body system is led to catastrophic collapse or
other obvious dynamical instability. Preliminary results (Figure
\ref{4.fig.1}) suggest the system does not exhibit catastrophic changes
within several inner-region dynamical times. However, there are
indications that the axial ratio $a:b$ in the inner region of the model
slowly increased from the initial value of $\approx 0.8$, suggesting that
the system is becoming more nearly axisymmetric. Nevertheless, at the
present time it is not clear whether this effect is real or just a
numerical artifact.


==> Chapters/dehnen.tex <==
\chapter{SELF-CONSISTENT MODELS OF TRIAXIAL DEHNEN ELLIPSOIDS}

This Chapter describes the use of Schwarzschild's numerical method for the
construction of self-consistent triaxial Dehnen ellipsoids. The principal
aim is to test the degeneracy of the solutions in terms of the range of
possible variations in the relative abundances of chaotic and regular
orbits populating the models.

\section{Motivation}
\label{3.sec.mot}

The role of chaos in the structure and dynamics of galaxies is an issue
still debated in the galactic community. While it is known that integrable
potentials form a set of measure zero in the space of potentials, there is
no {\it a priori} reason to exclude the possibility, however seemingly
far-fetched, that the mechanics of galaxy formation somehow favor (or lead
to) mass density distributions that generate integrable potentials, \eg
via some sort of feedback mechanism related to ``violent relaxation.''

A more fruitful way to approach the question of the role of chaos in
galaxies would arguably be to construct {\em self-consistent} models of
galaxies, as opposed to studying fixed potentials, for which one often
cannot know in advance whether they can be self-consistently supported via
Poisson's law. There are two known ways to construct self-consistent
models numerically: Schwarzschild's method (or variants thereof, aimed at
deconvolving phase-space DFs from observationally accessible quantities)
and $N$-body simulations, which are by definition self-consistent. Either
one is harder to implement and interpret than studies of fixed ``toy''
potentials (although, of course, such studies are still necessary as
precursors to the construction of a quality library of orbital templates
for use with Schwarzschild's method -- see the discussion in the previous
Chapter).

Unfortunately, neither Schwarzschild's technique nor $N$-body simulations
can offer an unequivocal answer to the initial question. Even if one
dismisses, for the moment, the numerical and conceptual problems
associated with Schwarzschild's method, one cannot ignore the fact that it
is not possible to know whether the form of the mass density distribution
$\rho(\xx)$ that is being used for the construction of the model actually
corresponds to something that exists in nature (just because it is
self-consistent does not necessarily mean it exists in nature!) This is so
because one cannot infer the three-dimensional $\rho(\xx)$ from
two-dimensional photometric observations (even assuming that the
mass-to-light ratio is known) unless some assumption is made about the
three-dimensional shape of the system. However, making a realistic
assumption may not be trivial, given the wealth of structural detail that
even elliptical galaxies often reveal upon closer inspection (isophotal
twists, boxiness, diskiness, varying ellipticities with radius, embedded
disks or other decoupled components, \etc). $N$-body simulations also
suffer from the same problem, which is further exacerbated by the
difficulty of defining and understanding chaos in $N$-body simulations and
how it relates to chaos in the collisionless Boltzmann
equation\footnote{Strictly speaking, there are strong indications, both
theoretical \citep{Kan90b} and numerical \citep{Mil64, KanSmi91, GooHeg93,
KanMah94b} that, at least for $N \gg 2$, {\em all} orbits in the generic
$N$-body problem are chaotic.}.

Nevertheless, in the absence of any known mechanism that would force
galactic potentials to become integrable, it seems legitimate to study the
effects of chaos on the structure and dynamics of galaxies. A desirable
by-product of such studies could be the identification of observable
effects that would be characteristic signatures of the presence of chaos
in galaxies. Within this framework, a study of self-consistent chaos is a
major step forward from the study of chaos in fixed potentials.

Shortly after \citet{Sch79} introduced his method for constructing
numerical equilibria, \citet{Mer80} realized that the time $t^o_c$ spent
by some orbits in the grid cells was different when they were integrated
on a different computer. Today this would be recognized as a telltale sign
of chaos, manifesting the fact that chaotic orbits exhibit an exponential
sensitivity to small changes of initial conditions, which can happen when,
\eg integration roundoff errors on different computers are different. This
was an early indication of the role of chaos in self-consistent models.
More recently, \citet{Kau93} and \citet{KauCon96} discovered that in order
to create self-consistent models of certain barred spiral galaxies,
chaotic orbits are required to fill the chaotic region near corotation,
where resonance overlap destroys regular motion.

\citet{MerFri96} presented what may be the strongest evidence yet that
chaos is required to construct self-consistent models of realistic
elliptical galaxies. They were motivated by recent Hubble Space Telescope
observations showing that most elliptical galaxies have central density
cusps $\rho(r) \sim r^{-\gamma}$, rather than extended cores, and also by
theoretical and numerical work suggesting that a central cusp or mass
concentration can induce chaos in a triaxial galaxy by destroying the
integrability of centrophilic box orbits (see \S\ref{1.sec.mot} for more
details). They used Schwarzschild's method to construct self-consistent
models of two triaxial ellipticals, one with a ``weak cusp'' and one a
``strong cusp,'' corresponding to $\gamma = 1$ and $2$, respectively. They
found that stochastic orbits contributed, respectively, 45\% and 60\% of
the total mass of the system. However, these models came with a caveat,
about which a few things should be said.

The construction of self-consistent models of nonintegrable systems
requires a generalization of Jean's theorem to include invariant
distributions of chaotic orbits as valid time-independent building blocks
\citep{Kan98}. For a potential that obeys only one classical integral,
namely the energy, the generation of the library of orbital templates has
to proceed in two steps. First, the regular orbits have to be sampled as
densely as possible and integrated for long enough until they populate
uniformly their invariant tori, in the spirit of the discussion in
\S\ref{2.sec.lib}. Secondly, one or more chaotic orbits have to be
integrated long enough until they uniformly populate the chaotic segments
of the constant-energy hypersurface. If one waits for long enough, one
single initial condition sampled anywhere in the chaotic region will
eventually (at the $t \to \infty$ limit) pass arbitrarily close to every
point in the chaotic regions of the hypersurface. In this sense, the
chaotic ``sea'' that surrounds the islands of regularity in a
nonintegrable system is filled by one single orbit. In practice, however,
it is usually more efficient to integrate several chaotic orbits, sampled
at different locations, and mix them (time-average their contributions to
the invariant measure). The reason why this is usually a better approach
is because chaotic regions in three-dimensional systems are interconnected
via the Arnold web, which can inhibit phase-space transport between
chaotic subdomains for very long times. If, however, more than one orbit
is integrated, chances are they will start in different chaotic
subdomains. The expectation then is that, even if none of them is
integrated long enough to escape its own subdomain, the time-averaged
distribution will be a better approximation to the invariant measure than
a single orbit integrated for as long as all them together.

There is some indirect evidence in support of this conjecture from
short-time Lyapunov exponent work. For example, in their analysis of
orbits in a truncated Toda potential, \citet{KanMah94} found that
computing short-time Lyapunov exponents for $n$ different initial
conditions, each integrated for a time $T$ and then averaging up, gave a
better approximation to the true Lyapunov exponent than integrating a
single initial condition for a much larger time $nT$.

\citeauthor{MerFri96} found that, when they insisted that their models be
constructed involving only fully mixed chaotic building blocks, no
self-consistent equilibria could be found. Instead, self-consistent models
could only be constructed if substantial portions of the chaotic orbits
were ``unmixed.'' For the weak-cusp $\gamma=1$ case, only the innermost
six shells could be mixed; for the strong-cusp $\gamma=2$ case, only the
innermost two.

In this Chapter, the same potential-density model used by \citet{MerFri96}
is re-examined in an attempt to independently test their results. There
are four main differences between the present implementation and the one
by \citeauthor{MerFri96}. First, a larger (by a factor of three) library
of orbits was used (20000 orbits instead of 6840); second, the library
sampling was slightly different; third, the orbits were integrated for
twice as long (200, instead of 100, dynamical times); fourth, chaotic
orbits were distinguished from regular orbits using a somewhat different
technique. A different optimization algorithm was also used, but other
than improved efficiency and robustness, this difference is not expected
to make any substantial difference. The question of
nonuniqueness/degeneracy was also addressed by searching for models which
both maximize and minimize the number of chaotic orbits.



\section{Density, Potential and Equations of Motion}

The mass density distribution that will be used is a triaxial
generalization of a class of spherical models studied by \citet{Deh93}:
\begin{equation}
  \rho(m) = \frac{(3-\gamma)M}{4\pi a b c} \, m^{-\gamma} \,
  (1+m)^{-(4-\gamma)}, \qquad 0 \le \gamma \le 3,
\end{equation}
where
\begin{equation}
  \label{3.eq.mu}
  m^2 = \frac{x^2}{a^2} + \frac{y^2}{b^2} + \frac{z^2}{c^2}, \qquad a \ge
  b \ge c \ge 0,
\end{equation}
and $M$ is the total mass. Mass is stratified on concentric ellipsoids
with axis ratios $a:b:c = 1.0:\sqrt{5/8} \approx 0.8:0.5$. The parameter
$\gamma$ determines the slope of the central density cusp. For $\gamma=0$
the model has a finite-density core; for $\gamma > 0$ the central density
is infinite. In the present work, the value $\gamma = 1$ will be used,
which corresponds to the weak-cusp model in \citet{MerFri96}.

The potential generated by this mass distribution for $\gamma \ne 2$ is
\begin{equation}
  \label{3.eq.pot}
  \Phi = -\frac{1}{2-\gamma} \int_0^1
  \frac{\{1-(3-\gamma)[m/(1+m)]^{2-\gamma} +
  (2-\gamma)[m/(1+m)^{3-\gamma}\} ds}{\sqrt{[1+(b^2-1)s^2][1+(c^2-1)s^2}},
\end{equation}
where
\begin{equation}
  m^2(s) = s^2 \left[x^2 + \frac{y^2}{1+(b^2-1)s^2} +
  \frac{z^2}{1+(c^2-1)s^2} \right].
\end{equation}
Finally, the accelerations are given by
\begin{equation}
  \label{3.eq.acc}
  \ddot{x_i} = -\frac{\ptl\Phi}{\ptl x_i} = -(3-\gamma)\frac{x_i}{a_i}
  \int_0^1 \frac{s^2 ds}{m_i^\gamma(1+m_i)^{4-\gamma}
  \sqrt{(a_i^2+A_1s^2)(a_i^2+A_2 s^2)}},
\end{equation}
where
\begin{equation}
  m_i^2(s) = s^2 \left( \frac{x^2}{a_i^2+C_1s^2} + \frac{y^2}{a_i^2+C_2s^2} +
  \frac{z^2}{a_i^2+C_3s^2} \right)
\end{equation}
and the constants are
\begin{eqnarray*}
  \mbox{for } i=1 & : & A_1=b^2-1, \quad A_2=c^2-1,
                      \quad C_1=0, \quad C_2=b^2-1, C_3=c^2-1 \\
  \mbox{for } i=2 & : & A_1=c^2-b^2, \quad A_2=1-b^2,
                      \quad C_1=1-b^2, \quad C_2=0, C_3=c^2-b^2 \\
  \mbox{for } i=3 & : & A_1=1-c^2, \quad A_2=b^2-c^2,
                      \quad C_1=1-c^2, \quad C_2=b^2-c^2, C_3=0
\end{eqnarray*}

The fact that the force depends on a nonanalytical integral makes the
orbit calculations very time consuming. It should also be noted here that
the two-dimensional projection of this mass distribution produces
isophotal ellipses that are concentric, twisted, and have constant
ellipticities. However, they do not exhibit any diskiness or boxiness.
Somewhat ironically, it would be less computationally expensive to use a
potential that {\em does} reproduce these features, but in the interest of
comparison with \citeauthor{MerFri96}, the same form for the potential is
retained for this work. However, it should be kept in mind that this
potential departs from axisymmetry only insomuch as to violate the
symmetry that conserves angular momentum.



\section{The Library of Orbits}
\label{3.sec.lib}

In order to generate initial conditions for the library of orbits, the
mass distribution is divided into 21 shells of equal mass using 20
isodensity surfaces. The value of the energy at the isopotential surface
tangent to each isodensity ellipsoid along the semi-major axis is then
computed.



\begin{figure}[hp]

\begin{center}
\epsfig{file=Figures/fig3-ic-a.eps,width=10cm}

\footnotesize{(a)}

\epsfig{file=Figures/fig3-ic-b.eps,width=10cm}

\footnotesize{(b)}

\end{center}
\caption{\label{3.fig.ic} The innermost octant of initial conditions for
the library of orbits of a triaxial Dehnen ellipsoid. (a) Sampling of the
stationary starting space (mostly box orbits). The initial conditions were
selected to be centered on segments of approximately equal area; (b)
Sampling of the principal planes (mostly tube orbits).}
\end{figure}



Following \citet{Sch93} and \citet{MerFri96}, the initial conditions are
sampled from two separate domains, in an attempt to maximize phase-space
coverage. The {\em stationary starting space} (Figure \ref{3.fig.ic}a) is
comprised of orbits with zero initial velocities and initial positions
sampled on the positive octant of each one of the 20 isopotential
surfaces. This was done in a fashion similar to the Plummer sphere
(\S\ref{2.sec.lib}), in other words so that each initial condition is
centered on approximately equal-area segments. The two main differences
from the Plummer case are that (i) the isopotential and isodensity
surfaces are not identical any more, so that one has to seek numerically
the intersection between the isopotential surface (given by
Eq.~(\ref{3.eq.pot}) in a nonclosed form) and the straight line joining
the center and a point on the isodensity surface; and (ii) the area
$\delta S(\delta\theta,\delta\phi)$ of a segment of an ellipsoid is not
available in a closed form, so that it, too, has to be computed
numerically from the second part of Eq.~(\ref{2.eq.deltaS}), where $r$ now
corresponds to $m$, given by Eq.~(\ref{3.eq.mu}). A total of 250 orbits
are sampled on every isopotential surface. Most are centrophilic box
orbits (Figure \ref{3.fig.orb3010}), and most are chaotic, presumably due
to their close passages to the center \citep{GerBin85}.

The {\em principal planes starting space} corresponds to orbits started on
the $x-y, x-z,$ and $y-z$ planes. A total of 250 orbits were sampled on
each plane, covering an annulus with an inner radius equal to the minimum
of the amplitudes of the 1:1 periodic orbits at that energy and on that
plane, and with an outer radius defined by the curve where the potential
is equal to the energy of the orbit (Figure \ref{3.fig.ic}b). The two
velocity components parallel to the principal plane were set to zero, and
the perpendicular component was computed from the energy with a positive
sign. Most of the orbits from the principal planes space are centrophobic
tube orbits (Figure \ref{3.fig.orb3330}), and most are regular.

A total of $3 \times 250 = 750$ principal planes initial conditions were
sampled at each energy level, which, together with the initial conditions
of the stationary starting space, defines 1000 orbits per energy level for
a grand total of 20000 orbits. Each orbit was integrated for a time equal
to 200 crossing times of the 1:1 periodic orbits of that energy. This
represents almost 3 times as many orbits integrated for twice as long as
in \citet{MerFri96}. Furthermore, these authors only used principal plane
initial conditions from the $x-y$ plane, whereas for this work, orbits
from all three planes were included, thus respecting better the symmetries
of the system.



\begin{figure}[t]
\begin{center}
\epsfig{file=Figures/fig3-enercons.eps,width=4in}
\end{center}
\caption{\label{3.fig.enercons} Absolute value of relative energy error
after an orbital integration of $\sim 200 \, t_{cr}$}
\end{figure}


\begin{figure}[p]

\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig3-orb3010-a.eps,width=7cm}
\footnotesize{(a)}
\end{center}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig3-orb3010-b.eps,width=7cm}
\footnotesize{(b)}
\end{center}
\end{minipage}

\vskip 1cm

\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig3-orb3010-c.eps,width=7cm}
\footnotesize{(c)}
\end{center}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\caption{\label{3.fig.orb3010} An example of a typical box orbit.}
\end{minipage}
\end{figure}


\begin{figure}[p]

\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig3-orb3330-a.eps,width=7cm}
\footnotesize{(a)}
\end{center}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig3-orb3330-b.eps,width=7cm}
\footnotesize{(b)}
\end{center}
\end{minipage}

\vskip 1cm

\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig3-orb3330-c.eps,width=7cm}
\footnotesize{(c)}
\end{center}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\caption{\label{3.fig.orb3330} An example of a typical loop orbit.}
\end{minipage}
\end{figure}


The same Bulirsch-Stoer method used for the integration of the Plummer
sphere orbits was also used for the triaxial Dehnen potential. The
integral in the acceleration equation (\ref{3.eq.acc}) was computed using
a 32nd-order Gauss-Legendre quadrature scheme. Energy conservation was
better than 1 part in $10^8$ for most but the highest-energy orbits
(Figure \ref{3.fig.enercons}). Poor energy conservation for these
high-energy orbits had to do with the much longer dynamical timescales in
the outer parts of the system, which led to longer real-time integrations,
as well as to the near-zero energies of the outermost orbits, which enter
the denominator of the relative energy error calculation. It would be
possible to improve energy conservation by using a higher order quadrature
scheme, but this was not deemed necessary for mainly two reasons: first,
improved orbital positions would not make a big difference at the level of
coarse-graining of the model; second, random numerical integration errors
act, in some sense, as noise, facilitating phase-space transport of
confined chaotic orbits, thus making these orbits more appropriate
time-independent building blocks.

Because regular and chaotic orbits need to be treated differently when
solving the optimization problem, it is important to be able to
distinguish between regular and chaotic orbits. For this reason, chaotic
orbits have to be identified first. This was done by calculating the
largest Lyapunov characteristic number $\chi$ associated with every orbit
(\S\ref{1.subsec.steady}). The numerical technique for evaluating $\chi$
was essentially a short-time implementation of Eq.~(\ref{1.eq.lyap}): for
every initial condition in the library, a ``companion'' initial condition
was created by perturbing the $x$ coordinate by $\delta x = 10^{-9}$. Both
initial conditions were actually evolved into the future, and the
companion orbit's phase-space distance from the primary orbit was
renormalized to $10^{-9}$ every dynamical time.


\section{The Coarse-Graining of Configuration Space}
\label{3.sec.grid}


\begin{figure}[t]
\begin{center}
\epsfig{file=Figures/fig3-grid.eps,width=4in}
\end{center}
\caption{\label{3.fig.grid} The grid used for the coarse-graining of
configuration space}
\end{figure}


The configuration-space grid used to solve the optimization problem is
similar to the one used for the Plummer sphere models. The only difference
is that the three segments are now defined by the planes $cx = az, cy =
zb,$ and $bx = ya$, to take into account the differing axis ratios of the
ellipsoid (Figure \ref{3.fig.grid}).


\section{The Optimization Problem}
\label{3.sec.optim}

As explained in \S\ref{3.sec.mot}, the presence of chaotic orbits
necessitates an alternative approach to computing DFs.  Specifically, the
chaotic orbits at every energy level have to be time-averaged and treated
as one single orbit, if the ensuing model is to represent a true
equilibrium. One good way to do that is using Pfenniger's technique,
outlined in \S\ref{2.sec.lib}. However, again in the interest of a
comparison with results obtained by \citet{MerFri96}, their approach was
used: once the library of orbital templates was computed, the chaotic
orbits were identified (see next paragraph), and their contributions to
each grid cell were added together and averaged out.

The identification of chaotic orbits was done differently from
\citeauthor{MerFri96}. For every energy level, the distribution of the
short-time Lyapunov exponents for the entire ensemble of 1000 orbits was
plotted (Figure \ref{3.fig.lyap}). The plots exhibit a bimodal
distribution: the low-$\chi$ component corresponds to orbits which are
either regular or confined chaotic, temporarily trapped near islands of
regularity. The high-$\chi$ orbits correspond to unconfined chaotic
orbits, populating the stochastic sea. An educated guess was made as to
the value of a critical $\chi = \chi_{crit}$ above which an orbit was
classified as chaotic. This classification scheme has the advantage that
it relies on ensembles of orbits, which make it easier to (i) identify how
high $\chi$ can be before an orbit has to be classified as chaotic (a
problem arising from the fact that only a short-time, $\chi(t \sim
200t_{cr})$, Lyapunov exponent and not the true $\chi(t \to \infty)$ limit
is actually computed), and (ii) determine whether there is a significant
component of confined chaotic orbits in the library (evidenced by a
bimodal shape in the distribution of high-$\chi$ orbits), which would
almost certainly lead to secular evolution. For each one of the 20 energy
levels, the occupation times $t^o_c$ of all chaotic orbits were averaged
up and were presented to the optimization software as a single orbit.


\begin{figure}[t]
\begin{center}
\epsfig{file=Figures/fig3-t14-res.eps,width=4in}
\end{center}
\caption{\label{3.fig.t14} Relative mass error $\sum_{o=1}^{N_o}
t^o_c w_o/m_c - 1$ as a function of cell number for an LP model of the
triaxial Dehnen potential where chaotic orbits are mixed up to 14th shell,
inclusive.}
\end{figure}


\begin{figure}[ph]
\epsfig{file=Figures/fig3-lyap-a.eps,width=6in}
\caption{\label{3.fig.lyap} The distribution of Lyapunov exponents far all
20 energy levels. The vertical dashed line represents the selected cutoff
value of $\chi$ that separates regular from chaotic orbits at every energy
level.}
\end{figure}

\begin{figure}[ph]
\epsfig{file=Figures/fig3-lyap-b.eps,width=6in}
\begin{center} Figure 3.7--continued \end{center}
\end{figure}

\begin{figure}[ph]
\epsfig{file=Figures/fig3-lyap-c.eps,width=6in}
\begin{center} Figure 3.7--continued \end{center}
\end{figure}

\begin{figure}[th]
\epsfig{file=Figures/fig3-lyap-d.eps,width=6in}
\begin{center} Figure 3.7--continued \end{center}
\end{figure}

The first question to ask is whether it is possible to have a
self-consistent model where the chaotic orbits at all 20 energy levels are
fully mixed, in the way described above. The answer is no. As shown in
Figure \ref{3.fig.t14}, if one enforces mixing up to, and including, shell
14, the deviations from self-consistency in several cells become high, and
the situation only gets worse as one increases the number of fully mixed
shells. It is only possible to fully mix up to 13 shells before the model
becomes infeasible.

The numerical DFs computed for the fully-mixed lower 13 shells included
four cases: One where the number of chaotic orbits was minimized (both
using LP and QP) and one where it was maximized (again, using LP and QP).
In the former case, $f(w_o)$ in Eq.~(\ref{2.eq.qp}) was given by
\begin{equation}
  f(w_o) = s \left( \sum_{\mbox{ch}} w_o - \sum_{\mbox{reg}} w_o \right)
\end{equation}
whereas in the latter by
\begin{equation}
  f(w_o) = s \left( \sum_{\mbox{reg}} w_o - \sum_{\mbox{ch}} w_o \right),
\end{equation}
where $s > 0$ is a coefficient and ``reg'' and ``ch'' correspond to
sums over regular and chaotic orbits, respectively.


The results are shown for all orbits in Figures \ref{3.fig.lminchaos} --
\ref{3.fig.qmaxchaos}, and for the chaotic orbits only in Figure
\ref{3.fig.wchaos}. The differences between the LP and QP approach are
marginal. However, there is a significant difference between the results
from the cost function that minimized the number of chaotic orbits and 
the cost function that maximized the number of chaotic orbits.
Specifically, the sum of the weights of the chaotic orbits in the first
case is $\approx 3.2 \times 10^{-5}$, compared to $\sim 0.08$ in the
second case. Therefore, there is some freedom in the number of chaotic
orbits that can populate the system. The maximum-chaos estimate places
about 8\% of the mass of the system in chaotic orbits, compared to 45\% in
\citet{MerFri96}. This discrepancy may be due to (i) differences in the
classification of confined chaotic orbits as regular or chaotic, or (ii)
the fact that the present work samples all three principal planes, instead
of only the $x-z$ plane, thus increasing the number of mostly regular loop
orbits.



\begin{figure}[p]

\vskip -6mm

\begin{center}

\epsfig{file=Figures/fig3-lminchaos-w.eps,width=9cm}

\footnotesize{(a)}

\epsfig{file=Figures/fig3-lminchaos-wdistr.eps,width=9cm}

\footnotesize{(b)}

\epsfig{file=Figures/fig3-lminchaos-res.eps,width=9cm}

\footnotesize{(c)}

\caption{\label{3.fig.lminchaos} Minimization of chaotic orbits -- LP
model (only the lower 13 shells are mixed). (a) Distribution of weights as
a function of orbit number; (b) Frequency distribution of orbital weights;
(c) Relative mass error $\sum_{o=1}^{N_o} t^o_c w_o/m_c - 1$ as a function
of cell number.}

\end{center}
\end{figure}


\begin{figure}[p]

\vskip -6mm

\begin{center}

\epsfig{file=Figures/fig3-qminchaos-w.eps,width=9cm}

\footnotesize{(a)}

\epsfig{file=Figures/fig3-qminchaos-wdistr.eps,width=9cm}

\footnotesize{(b)}

\epsfig{file=Figures/fig3-qminchaos-res.eps,width=9cm}

\footnotesize{(c)}

\caption{\label{3.fig.qminchaos} Minimization of chaotic orbits -- QP
model (only the lower 13 shells are mixed). (a) Distribution of weights as
a function of orbit number; (b) Frequency distribution of orbital weights;
(c) Relative mass error $\sum_{o=1}^{N_o} t^o_c w_o/m_c - 1$ as a function
of cell number.}

\end{center}
\end{figure}


\begin{figure}[p]

\vskip -6mm

\begin{center}

\epsfig{file=Figures/fig3-lmaxchaos-w.eps,width=9cm}

\footnotesize{(a)}

\epsfig{file=Figures/fig3-lmaxchaos-wdistr.eps,width=9cm}

\footnotesize{(b)}

\epsfig{file=Figures/fig3-lmaxchaos-res.eps,width=9cm}

\footnotesize{(c)}

\caption{\label{3.fig.lmaxchaos} Maximization of chaotic orbits -- LP
model (only the lower 13 shells are mixed). (a) Distribution of weights as
a function of orbit number; (b) Frequency distribution of orbital weights;
(c) Relative mass error $\sum_{o=1}^{N_o} t^o_c w_o/m_c - 1$ as a function
of cell number.}

\end{center}
\end{figure}




\begin{figure}[p]

\vskip -6mm

\begin{center}

\epsfig{file=Figures/fig3-qmaxchaos-w.eps,width=9cm}

\footnotesize{(a)}

\epsfig{file=Figures/fig3-qmaxchaos-wdistr.eps,width=9cm}

\footnotesize{(b)}

\epsfig{file=Figures/fig3-qmaxchaos-res.eps,width=9cm}

\footnotesize{(c)}

\caption{\label{3.fig.qmaxchaos} Maximization of chaotic orbits -- QP
model (only the lower 13 shells are mixed). (a) Distribution of weights as
a function of orbit number; (b) Frequency distribution of orbital weights;
(c) Relative mass error $\sum_{o=1}^{N_o} t^o_c w_o/m_c - 1$ as a function
of cell number.}

\end{center}
\end{figure}



\begin{figure}[p]

\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig3-lminchaos-wchaos.eps,width=7cm}
\footnotesize{(a)}
\end{center}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig3-qminchaos-wchaos.eps,width=7cm}
\footnotesize{(b)}
\end{center}
\end{minipage}

\vskip 1cm

\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig3-lmaxchaos-wchaos.eps,width=7cm}
\footnotesize{(c)}
\end{center}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig3-qmaxchaos-wchaos.eps,width=7cm}
\footnotesize{(b)}
\end{center}
\end{minipage}

\caption{\label{3.fig.wchaos} Distribution of weights for the 13 chaotic
orbit templates. (a) Minimization of chaotic orbits -- LP model; (b)
Minimization of chaotic orbits -- QP model; (c) Maximization of chaotic
orbits -- LP model; (d) Maximization of chaotic orbits -- QP model.}

\end{figure}


==> Chapters/introduction.tex <==
\chapter{INTRODUCTION AND MOTIVATION}

\section{Some Preliminaries about Galaxies}
\label{1.sec.prelim}

The research field of galactic dynamics was arguably born when Edwin
Hubble established in 1923 that William Parsons' ``spiral nebulae,'' a
subset of objects from William Herschel's extensive catalog of nebulae,
were in fact gigantic conglomerations of stars, like the Milky Way galaxy.
They were thus appropriately called ``galaxies,'' and the Milky Way was
demoted to a mere sample in a universe filled with billions of peer
galaxies -- though its initial letter was now capitalized and promoted to
``the Galaxy.'' Most galaxies lie at such enormous distances that only the
combined glow of their billions of stars can be detected. This explains
why, until 75 years ago, they were confused with the visually similar soft
glow of emission nebulae in the Galaxy.

Galaxies come in a variety of shapes, sizes and masses. In terms of their
appearance, they are classified as spiral, elliptical and irregular, based
on the morphological classification scheme introduced by \citet{Hub36}.
Spiral galaxies come in two flavors, normal and barred (although there is
mounting evidence that most spirals are barred, with only the size of the
bar varying among them). In order of increasing tightness of the winding
of their spiral arms, spirals are classified as S(B)c, S(B)b or S(B)a, as
well as S(B)0 (or lenticular) when they exhibit a central bulge but no
identifiable spiral arms. The letter B is included when the spiral is
barred.

Ellipticals are designated E$n$, where $n = 10[1-(b/a)]$ and $b/a$ is the
axial ratio of their projected brightness ellipsoid. The index $n$ ranges
from 0 for round ellipticals to 6 for highly elongated ones. Very few, if
any, ellipticals are more elongated than E6, for reasons that seem to be
related to dynamical instabilities that grow with increasing ellipticity
\citep[\cfeg][]{MerSti90, MerHer91}. It should be noted that, whereas the
spiral sequence S0-Sa-Sb-Sc correlates, at least roughly, with significant
physical quantities (for instance, the importance of dynamical rotation
increases, compared to random motions, from S0 to Sc), this does not seem
to be the case with the elliptical E0-E6 sequence, where variations in
apparent ellipticities must be mainly a result of projection effects.
However, one can still extract some important conclusions from the {\em
statistical} manipulation of the projected axial ratios of elliptical
galaxies.

It is useful to keep in mind that the E$n$ subclassification scheme is not
as well-defined and consistent as one might think, mainly due to
inadequacies of the photographic techniques that were used for the
classification of most elliptical galaxies. For example, different workers
used the axis ratios of different isophotes to determine $n$. Furthermore,
more detailed observations have revealed quite early on that {\it the
ellipticity of the isophotes can change with radius}
\citep[\cfeg][]{RedShi38, Lil60, Lil66, Car78}, leading to the
inconvenience that the subclassification of a given elliptical may change
as a function of the position, along the semimajor axis, where the
ellipticity is determined. Therefore, the index $n$ should only be taken
as a visual indication of ellipticity measured at a ``moderately faint''
isophote.

Another effect that is not taken into account in the E$n$
subclassification is the occurrence of {\it isophote twists}, \ie
variations with radius of the position angles of the major axes of the
isophotes. Evidence for this effect, which is present in many ellipticals,
started accumulating early on \citep[\cfeg][]{Eva51, Lil60, Car78,
WilSch79}. Both variations in ellipticity and in position angle were
confirmed and studied in detail with subsequent CCD observations.

More recently \citep{KorBen96, TreMer96}, some consensus seems to be
developing among workers that, based on physically significant criteria,
most elliptical galaxies fall into one of two categories. In the first
category belong normal- and low-luminosity, rapidly rotating, nearly
isotropic, oblate-spheroidal ellipticals, which can be morphologically
distinguished for being coreless and for having {\em disky-distorted
isophotes}. In the second category belong giant, essentially non-rotating,
anisotropic and moderately triaxial ellipticals that have cuspy cores and
{\em boxy-distorted isophotes} (by ``triaxial'' these authors mean that
the equidensity surfaces in the outer parts of the galaxies are
non-degenerate ellipsoids, \ie ellipsoids with three different semi-axes
$a > b > c$; see  \S\ref{1.sec.mot.triax} for more on triaxiality and
elliptical galaxies). This dichotomy, if true, could also imply different
formation processes for the two categories of ellipticals. For example, it
is tempting to suggest that triaxial slow rotators are the remnants of
galactic mergers, whereas the spheroidal, flattened, fast rotators formed
via dissipative processes and are perhaps continuously linked to the S0
type of disk galaxies that show no spiral structure.

Concerning now the masses of galaxies, if the galaxian mass distribution
in the Local Group of galaxies is typical, then dwarf galaxies with masses
$M \sim 10^6-10^{10} M_\odot$ (such as the irregular Magellanic Clouds, or
M32, the dwarf elliptical companion of the Andromeda galaxy) should
outnumber the normal galaxies with $M \sim 10^{11} - 10^{12} M_\odot$
(such as the Galaxy and M31, the Andromeda galaxy) by at least an order of
magnitude. The most massive galaxies ($M \sim 10^{13} M_\odot$) are the
central dominant (cD) galaxies that reside near the centers of many
clusters of galaxies. Notwithstanding the sheer numbers of dwarf galaxies
and the large masses of cD galaxies, most of the luminous mass in the
local universe probably resides in normal galaxies.

The luminous matter in galaxies consists mainly of stars, gas and dust.
Stars are responsible for the overwhelming fraction of the luminous  mass
of most galaxies. In spiral galaxies, the contribution of gas and dust to
the total mass is usually restricted to the few-percent level, although in
some rare cases it can account for up to 10-20\%. It might thus seem that,
at least as far as dynamics is concerned, gas and dust play a marginal
role for all but the most gas-rich spirals. Indeed, they are often treated
as test particles, moving under the influence of the stellar gravitational
background field.

However, this picture is not entirely accurate. Despite their relative
sparsity, gas and dust play an essential role in star formation, the
evolution of bars, the formation of spiral arms, and in other processes
that rely on the dissipative properties of gas. The capability of gas to
convert organized kinetic energy into random thermal motion via
dissipation enables it to go to places where stars cannot go, because they
are subject to Liouville's theorem and their motion is restricted by the
incompressibility of Hamiltonian flows. Gas can thus alter the mass
distribution of a spiral galaxy over time and cause secular evolution.
Furthermore, clumpy gaseous structures, such as giant molecular clouds,
often present fairly substantial gravitational cross-sections that can
scatter stars much more effectively than star-star encounters, thus
``heating'' disk stars (\ie increasing the velocity dispersion of the disk
population) and accelerating phase-space transport. The upshot is that,
depending on the particular problem at hand, it may or may not  be safe to
ignore gas in a dynamical study of spiral galaxies.

The situation is quite different for elliptical galaxies. Until less than
two decades ago, it was widely believed, on the basis of optical
observations, that ellipticals contain very little gas and dust. Since
then, X-ray observations have established the presence of substantial
amounts of {\em hot} ($\sim 10^7$ K) gas \citep[\cfeg][and references
therein]{Fab89}. In fact, the gas-to-star mass ratio in ellipticals seems
to be comparable to that in spirals, though in the latter it is found
mostly in warm ($\sim 10^4$ K ionized gas) and cold ($ < 100$ K atomic and
molecular gas) conditions. Ellipticals also contain warm and cold gas, as
well as dust, but their quantities are almost negligible. In fact, most
cases of substantial warm/cold gas and/or dust detections have been
reported for ellipticals that are morphologically classified as peculiar.
Furthermore, in these cases, the cold gas and dust often appear to be
kinematically decoupled from the stellar population. This evidence
suggests that cold gas and dust must have an external origin, such as
mergers with gas-rich companion galaxies \citep[\cfeg][and references
therein]{BreHog92}.

Despite the fact that elliptical galaxies possess a rich and complex
interstellar medium, which is still not very well understood, its effect
on the dynamics of its host galaxy is expected to be all but negligible,
given the low fraction of the total mass that it represents. Furthermore,
the Jeans mass associated with gas at such high temperatures is so large
that gas cannot collapse to form stars. In general, the high virial
temperature of the gas prevents it from forming clumps and substructures
that could affect the dynamics of ellipticals in ways similar to the ones
described above for spirals. Instead, the interstellar gas of elliptical
galaxies acts more like a backdrop against which stellar dynamics unfolds,
and is therefore safe to ignore in most dynamical studies.

The preceding discussion concerned the {\em luminous} matter in galaxies
and ignored their content in {\em dark} matter, the purported substance
out of which as much as 90-99\% (or even more, according to some
estimates) of the mass of the universe is made, but which emits no
detectable electromagnetic radiation. Its presence is only inferred from
its gravitational effects on visible matter. These effects are most
important over cosmological and intergalactic distance scales, although
they can also affect the internal dynamics of galaxies. For example, the
presence of massive dark halos surrounding disk galaxies may play a major
role in the formation and strength of disk warps, bars and other
structures. The effects of dark matter on elliptical galaxies are less
clear \citep[\cfeg][]{StiSpa91}.

Nevertheless, the very fact that dark matter emits no detectable amounts
of electromagnetic radiation strongly suggests that it is non-dissipative
in nature. This, in turn, implies that (a) it clumps less than luminous
matter, and thus it might not dominate the dynamics of galaxies that
presumably live near the bottom of the gravitational well created by the
dark matter, and (b) to the extent that dark matter does influence the
dynamics of luminous matter, at least the dynamics is still Hamiltonian.
In other words, if one assumes galactic matter is collisionless, whether
it is dark matter or stars is nearly irrelevant.

The research presented in this dissertation was conducted without taking
dark matter into account. This was done not because it is dynamically
unimportant, although for the kind of questions posed here it may well be,
but (i) because current understanding of the dark matter problem is quite
incomplete, thus making it hard to correctly incorporate it in this
dynamical study; and, more importantly, (ii) because the aim of this work,
as explained in \S\ref{1.sec.mot}, is to develop a better understanding of
certain generic physical processes that may be taking place in elliptical
galaxies, irrespective, to a certain extent, of the specific form of their
gravitational potentials --so long as the collisionless, Hamiltonian
approximation remains valid. For the same reason, no reference will be
made to the effects of varying mass-to-light ratios, which {\em can} be
important if one studies the dynamics of a {\em specific} object. However,
there is still a potential concern, namely that stars and dark matter
could evolve differently as they approach equilibrium, especially if the
dark matter is made of very low-mass fermions which cannot clump on short
scales. But allowing for such degeneracy is outside the scope of this
work.

Finally, it should be noted that the preceding discussion refers to
galaxies in the {\em local} universe. At times that correspond to
redshifts of $z > 2$ or so, most of the matter in galaxies was still in
the form of gas, and gas dynamics played a much more important role.
Peculiar and irregular galaxies were more common and, especially at still
higher $z$'s, galactic collisions were more common as well. A
collisionless, nearly-time-independent approach to galactic dynamics would
presumably not be particularly fruitful at those times.

The following section is a brief overview of the mean field theory and the
collisionless Boltzmann equation, the foundations for the statistical
treatment of dissipationless self-gravitating systems of many bodies.
Solving the collisionless Boltzmann equation is the topic of
\S\ref{1.sec.solve_CBE}, followed by a discussion of the outstanding
problems that motivated this work and an overview of the dissertation in
\S\ref{1.sec.mot}.



\section{The Collisionless Boltzmann Equation and the Mean Field
Approximation}
\label{1.sec.cbe}

Let the probability of a given ensemble of $N$ stars, that represents the
density distribution of a galaxy, at a given time $t$ be
\begin{equation}
  \mu \equiv \mu(\xx_1, \pp_1, \ldots, \xx_i, \pp_i, \ldots, \xx_N, \pp_N, t),
\end{equation}
so that $\mu \, d\Gamma$, where $d\Gamma \equiv \prod\limits_{i=1}^{N}
d\Gamma_i \equiv \prod\limits_{i=1}^{N} d^3\xx_i \, d^3\pp_i$, represents
the joint probability that star $i$ be found inside the phase-space volume
element  centered around $(\xx_i, \pp_i)$, simultaneously for all $i = 1,
\ldots N$ at time $t$. This implies that $\mu$ is normalized so that
$\int\mu \, d\Gamma = 1$, which is feasible since it is a realistic
expectation for galaxies that $\mu \to 0$ as $|\xx_i|$ and $|\pp_i| \to
\infty$ (there is a finite number of stars in a galaxy).

If there are no sources or drains of stars in the system, then
conservation of probability and the incompressibility of the flow dictate
that
\begin{equation}
  \frac{d\mu}{dt} \equiv \frac{\ptl\mu}{\ptl t} +
                  \left( \sum_{i=1}^{N}  \frac{\ptl\mu}{\ptl\xx_i} \cdot
                                         \frac{d\xx_i}{dt} \right) +
                  \left( \sum_{i=1}^{N}  \frac{\ptl\mu}{\ptl\pp_i} \cdot
                                         \frac{d\pp_i}{dt} \right)
                         = 0,
\label{1.eq.mu}
\end{equation}
where $\ptl / \ptl \xx \equiv (\ptl / \ptl x) \hat{\imath} + (\ptl / \ptl
y) \hat{\jmath} + (\ptl / \ptl z) \hat{k}$ for any vector $\xx$, and
$\cdot$ denotes the inner product. However, from the equations of motion
for a self-gravitating system of point masses one obtains
\begin{equation}
  \frac{d\xx_i}{dt} = \frac{\pp_i}{m}
\label{1.eq.mot1}
\end{equation}
and
\begin{equation}
  \frac{d\pp_i}{dt} =
         - \sum_{i = 1 \atop i \not= j}^N \frac{\ptl V(i,j)}{\ptl\xx_i} \equiv
         - \sum_{i = 1 \atop i \not= j}^N \frac{\ptl}{\ptl\xx_i}
                        \left( \frac{Gm^2}{|\xx_i - \xx_j|} \right),
\label{1.eq.mot2}
\end{equation}
where $V(i,j)$ is the two-body potential, and $m$ is the mass of
individual stars in the system, which is assumed to be the same for all
stars. This assumption imparts no loss of generality within the context of
a mean field approximation (see below in this section), where stars are
treated as zero-mass test particles moving under the influence of the bulk
field.

Even though $\mu$ is the fundamental statistical object, it is an
$N$-particle distribution function (DF) that cannot be directly compared
to any observables. Of more interest in that respect would be the
one-particle DF
\begin{equation}
  f(\xx_i,\pp_i,t) \equiv f(i) =
  \int \mu \, d\Gamma_1 \ldots d\Gamma_{i-1} \, d\Gamma_{i+1} \ldots d\Gamma_N
\label{1.eq.f1}
\end{equation}
that provides the probability of finding particle $i$ near
$(\xx_i,\pp_i)$, irrespective of the positions and velocities of the other
stars in the system. Substitution of Eqs.~(\ref{1.eq.mu}),
(\ref{1.eq.mot1}) and (\ref{1.eq.mot2}) into (\ref{1.eq.f1}) and
integration by parts (remembering that $\mu \to 0$ as $|\xx_i|$ and
$|\pp_i| \to \infty$ and that all particles are assumed to be identical)
gives
\begin{equation}
  \frac{\ptl f(i)}{\ptl t} +
  \frac{\pp_i}{m} \cdot \frac{\ptl f(i)}{\ptl \xx_i} -
  (N - 1) \, \frac{\ptl}{\ptl \pp_i} \cdot
          \int d\Gamma_j \, \frac{\ptl V(i,j)}{\ptl \xx_i} \, g(i,j) = 0,
\label{1.eq.boltz}
\end{equation}
where
\begin{equation}
  g(i,j) \equiv g(\xx_i, \pp_i, \xx_j, \pp_j, t) =
  \int \mu \, d\Gamma_1 \ldots d\Gamma_{i-1} d\Gamma_{i+1}
                        \ldots d\Gamma_{j-1} d\Gamma_{j+1} \ldots
                        d\Gamma_N
\end{equation}
is the two-particle DF. In other words, the evolution of the one-particle
DF requires knowledge of the two-particle DF, and in general the evolution
of the $n$-particle DF requires knowledge of the $(n+1)$-particle DF, all
the way up to $N$ (BBGKY hierarchy). This inability to decouple local from
global dynamics is a consequence of gravity being a long-range force. Some
progress can be made by writing
\begin{equation}
  g(i,j) = f(i) f(j) + \gamma(i,j),
\label{1.eq.corr}
\end{equation}
where $\gamma(i,j)$ reflects the degree to which stars $i$ and $j$ are
correlated. In general, $\gamma(i,j) \not= 0$, \ie the probability of
finding particle $i$ near $(\xx_i,\pp_i)$ depends on the probability of
finding particle $j$ near $(\xx_j,\pp_j)$. Substitution of Eq.~
(\ref{1.eq.corr}) into (\ref{1.eq.boltz}) yields
\begin{equation}
  \frac{\ptl f(i)}{\ptl t} +
  \frac{\pp_i}{m} \cdot \frac{\ptl f(i)}{\ptl \xx_i} -
  \frac{\ptl \bar{V}(i)}{\ptl \xx_i} \cdot \frac{\ptl f(i)}{\ptl \pp_i} =
  (N - 1) \, \frac{\ptl}{\ptl \pp_i} \cdot
          \int d\Gamma_j \, \frac{\ptl V(i,j)}{\ptl \xx_i} \, \gamma(i,j),
\label{1.eq.boltz2}
\end{equation}
where
\begin{equation}
  \bar{V}(i) \equiv \bar{V}(\xx_i,t) = (N-1) \int d\Gamma_j \, f(j) V(i,j)
\end{equation}
is the mean potential energy associated with the average forces acting on
particle $i$, and the right hand side describes the evolution of the
one-particle DF caused by particle-particle correlations.

If it is valid to approximate $\gamma(i,j) \approx 0$, then
Eq.~(\ref{1.eq.boltz2}) becomes the {\em collisionless Boltzmann equation
(CBE)} \citep[also known as the {\em Vlasov equation} in plasma physics,
but see as well][]{Hen82}:
\begin{equation}
  \frac{\ptl f}{\ptl t} +
  \vv \cdot \frac{\ptl f}{\ptl \xx} -
  \frac{\ptl \Phi}{\ptl \xx} \cdot \frac{\ptl f}{\ptl \pp} = 0,
\label{1.eq.CBE}
\end{equation}
where the indices have been dropped for convenience since all the
particles are considered to be identical, $\vv \equiv \pp/m$ is the
velocity of the particle, and
\begin{equation}
  \Phi(\xx,t) \equiv \frac{\bar{V}(\xx,t)}{N} \approx
                     \frac{\bar{V}(\xx,t)}{N-1} =
                -Gm^2 \int \frac{f(\xx',\vv',t)}{|\xx-\xx'|} \, d\Gamma'
\end{equation}
is the potential energy (this implies the normalization $\int f \, d\Gamma
= N$).

Setting $\gamma(i,j) = 0$ is called the {\em self-consistent field
approximation}. This {\em mean field theory} approach, that led to the
CBE, is a conceptually important tool that enables the worker to neglect
direct particle-particle interactions, which can be hard to model, and
describe the evolution of a particle solely as a result of its interaction
with the bulk gravitational field. The most important consequence of this
simplification stems from the fact that the CBE can be shown to be a
(noncanonical) Hamiltonian system, ${\cal H}[f]$, where the fundamental
variable is $f$ itself and ${\cal H}[f]$ represents the mean field energy
\citep{Mor80, Kan90}:
\begin{equation}
  {\cal H}[f] = \frac{1}{2} \int d^3\xx \, d^3\vv \, v^2 f(\xx,\vv,t) -
                \frac{G}{2} \int d^3\xx \, d^3\vv
                \int d^3\xx' \, d^3\vv' \,
                \frac{f(\xx,\vv,t) \, f(\xx',\vv',t)}{|\xx-\xx'|}.
\end{equation}
Clearly, then, it is important to investigate whether and when the
assumption that $\gamma(i,j) = 0$ is a valid and realistic approximation.

\citet{Cha43a}, in his classic monograph ``Principles of Stellar
Dynamics,'' considered the gravitational Rutherford scattering of a test
star moving in an idealized infinite and homogeneous distribution of point
stars. By symmetry, there is no net force acting on the test star due to
the bulk gravitational field of the system, so that, in the absence of
``close'' encounters with other stars, it would simply move at a constant
velocity. However, random stellar encounters do occur and they have the
effect of altering the velocity and the energy of the test star. In a real
galaxy all stars obviously participate in this process, which leads to a
secular evolution towards, albeit not to, a ``relaxed'' state of local
thermodynamic equilibrium, characterized by a Maxwellian, isothermal
distribution of stellar velocities \citep{Kan85}. The {\em relaxation
time}, $t_R$, is then defined as the time needed for the cumulative
effects of stellar encounters to alter the orbit of the test star to such
an extent that the mean field approximation breaks down, meaning that the
star cannot be considered as an independent, conservative dynamical system
any more. This could be quantified, for example, by the time needed for
the root-mean-square (rms) energy changes suffered by the test star as a
result of the encounters to become comparable to its total energy.

An alternative approach, also pioneered by \citet{Cha43b}, treats stellar
encounters as a stochastic process, and is a typical example of the {\em
fluctuation-dissipation} theorem. There are three ingredients in this
picture:
\begin{itemize}

\item The bulk gravitational potential, $\Phi$, that determines the motion
in the absence of any stellar encounters.

\item A systematic {\em diffusion} in velocity space, modeled as a sum of
``random kicks'' experienced by the test star due to its encounters with
other stars. These can be seen as random force ($\mathbf F$) fluctuations
overimposed to the bulk mean field. They have the effect of pumping
kinetic energy into the test star by increasing its rms velocity. $\mathbf
F$ is usually idealized as a delta-correlated Gaussian random process with
zero mean ($\langle \mathbf F \rangle = 0$). Delta-correlation means that
the forces at times $t_1$ and $t_2$ are uncorrelated, whereas Gaussian
statistics means that the process is characterized  completely by its
first two moments. Therefore, everything about $\mathbf F$ is encapsulated
in the two-point correlation function $ \langle \, {\mathbf F}^i(t_1) \,
{\mathbf F}^j(t_2) \, \rangle \propto \delta^{ij} \, \delta(t_1-t_2)$,
where the superscripts $i,j$ indicate spatial components, and the terms
$\delta(t_1-t_2)$ and $\delta^{ij}$ respectively express the fact that the
force is time-uncorrelated, and that its vector components in different
directions are also uncorrelated. The proportionality coefficient will be
specified below.

\item A systematic {\em dynamical friction}, $-\eta\vv$, antiparallel to
the direction of motion, that has the effect of continuously decelerating
the test star along its direction of motion. Dynamical friction can be
understood qualitatively by considering the test star moving with velocity
$\vv$ in the surrounding medium and creating a ``wake'' of stars behind
it. The wake corresponds to an excess density of stars behind the moving
test star, and the gravitational force associated with it will tend to
decelerate the test star along its direction of motion. In other words,
dynamical friction has the effect of removing kinetic energy from the test
star and heating up the surrounding medium. The coefficient $\eta$, which
has units of inverse time (see~Eq.~\ref{1.eq.langevin} below), scales as
$\eta \sim t_R^{-1}$, This is not surprising since both $\eta$ and $t_R$
reflect the effects of graininess induced by the fluctuations and should
be characterized by similar time scales.

\end{itemize}
These three ingredients interact according to a Langevin-type equation:
\begin{equation}
  \frac{d\rr}{dt} = \vv \qquad \mbox{and} \qquad \frac{d\vv}{dt} =
                    - \nabla\Phi - \eta\vv + \mathbf{F},
\label{1.eq.langevin}
\end{equation}
where, from the preceding discussion, it follows that the random force
$\mathbf F$ must obey
\begin{equation}
  \langle \mathbf F \rangle = 0 \qquad \mbox{and} \qquad
  \langle \, {\mathbf F}^i(t_1) \, {\mathbf F}^j(t_2) \,
  \rangle = 2 \, \eta \, \Theta \, \delta^{ij} \, \delta(t_1-t_2).
\end{equation}
Here $\Theta$ is the characteristic temperature (or mean squared velocity)
associated with~$\mathbf F$.

It is important to assess the effects of collisionality in the study of
stellar systems: considering the complications introduced by taking it
into account, it would be useful to see if there are cases where it can be
dismissed. The first question to ask then is what the time scale of
relaxation is. From the preceding discussion it becomes apparent that
there are a number of ways for defining $t_R$, but they are all associated
by the same physical process and, quite reassuringly, they all lead to the
same functional form and similar numerical values for $t_R$
\citep{Cha43a}:

\begin{equation}
  t_R \approx \frac{0.1\bar{v}^3 R^3}{G^2 m^2 N \ln N},
\end{equation}
where $\bar{v}$ is the characteristic stellar speed, $R$ is the
characteristic size of the system, and $N$ is the number of stars it
contains. If the system is in approximate virial equilibrium, then
$\bar{v}^2 \approx (GNm)/R$, in which case the last equation becomes
\begin{equation}
  t_R \sim \frac{N}{\ln N} \, t_D,
\end{equation}
where $t_D \sim R/\bar{v}$ is a typical dynamical, or crossing, time for
the system. 

The second question to ask is how important collisionality is in a
realistic stellar system. In the case of relatively small stellar systems,
such as globular clusters with $N \sim 10^5$ stars and $t_D \sim 10^5$ yr,
stellar collisions may be important over a cluster's typical lifetime of
$\sim 10^{10}$ yr. However, for galaxies with $N \sim 10^{11}$ stars and
$t_D \sim 10^8$ years, the relaxation time is several orders of magnitude
longer than the age of the universe. This has been customarily interpreted
\citep[\cfeg][p.\ 190]{BinTre87} as implying that stellar encounters are
entirely unimportant and that the collisionless Boltzmann equation is an
adequate description of the dynamics. However, this may not always be the
case and collisional effects may be important in relation to the question
of structural stability of galaxies \citep{Pfe86, HabKan97}.


\section{Solving the Collisionless Boltzmann Equation}
\label{1.sec.solve_CBE}

\vskip 5mm

\subsection{Time-Dependent Solutions}

\underline{\smash{Analytical solutions.}} The time-dependent CBE
(\ref{1.eq.CBE}) is a seven-dimensional partial differential equation.
Generic analytical solutions are only known for highly idealized systems,
systems of lower dimensionality and for special cases \citep[\cfeg][and
references therein]{Tal75, LouGer88, Sri89, CarSolVaz97, Dav90} 

However, it is still possible to extract useful information from the CBE
analytically, by calculating moments of the equation. Thus, for example,
by integrating Eq.~(\ref{1.eq.CBE}) over all possible velocities one
obtains the zeroth-order moment, which is a {\em continuity equation} in
configuration space:
\begin{equation}
  \frac{\ptl\rho}{\ptl t} + \frac{\ptl(\rho\bar{v}_i)}{\ptl x_i} = 0,
\end{equation}
where $\rho(\xx)$ is the configuration-space density of the system and
$\bar{v}_i(\xx)$ is the mean value of the $i-$th component of the
velocity. Similarly, by multiplying Eq.~(\ref{1.eq.CBE}) by $v_i$ and
integrating over all velocities, one obtains the first-order moment, which
is the analog of {\em Euler's equation} for stellar dynamics:
\begin{equation}
  \rho \, \frac{\ptl\bar{v}_i}{\ptl t} +
  \rho\bar{v}_j \, \frac{\ptl\bar{v}_i}{\ptl x_j} +
  \frac{\ptl(\rho\sigma_{ij}^2)}{\ptl x_j} +
  \rho \, \frac{\ptl\Phi}{\ptl x_i} = 0,
\end{equation}
where $\rho \sigma_{ij}^2 \equiv \rho (\overline{v_i v_j} - \bar{v}_i
\bar{v}_j)$ is the symmetric stress tensor, the analog of pressure ($p \,
\delta_{ij}$) for fluids. The utility of these two relations, which are
called the {\em Jeans equations}, should now be obvious: even though they
contain less information than the CBE itself, they describe observable
quantities, such as density, mean velocity and velocity dispersions, thus
enabling, at least in principle, comparison with observations (\cf
\S\ref{1.subsec.steady}). A number of problems in stellar dynamics have
been addressed via the Jeans equations \citep[\cfeg][pp.\ 198 -
211]{BinTre87}.

There is no reason why higher order moments cannot be computed. In fact,
it might at first seem possible to distill much of the information
contained in the CBE by considering a coupled set of moments equations,
truncated to some appropriately high order. This is indeed a viable option
(see ``numerical solutions'' below) but it turns out that every moment
equation of a given order contains dispersion terms that can only be
computed by a moment equation of the next higher order (for example,
$\sigma_{ij}^2$ involves $\overline{v_i v_j}$ that can only be computed
via a second-order moment equation). This is unlike the case with fluid
dynamics, where an equation of state, $p = p(\rho)$, allows one to
truncate the hierarchy by providing a relation between local pressure and
density. Such an equation of state reflects the fact that perfect fluids
are collision-dominated, so that one can assume local thermal equilibrium.
By contrast, self-gravitating systems like galaxies are presumed to be
nearly collisionless (this is why, for example, it makes sense to identify
an anisotropic pressure tensor for equilibrium solutions to the CBE). Thus
an infinite system of moment equations is needed to describe all the
information contained in the CBE. However, it is still possible to make
use of moment equations by truncating the infinite series via some
assumption about the form of $\sigma_{ij}^2$. Obviously, the validity of
this approximation depends on the validity of the assumption.

\underline{\smash{Numerical solutions.}} In order to study more realistic
systems one has to resort to numerical simulations. Unfortunately, solving
the full-fledged seven-dimensional equation is so taxing in terms of
computer speed and, even more so, memory requirements that only very
recently is it becoming feasible to use grids that are large enough to
attack realistic problems in three degrees of freedom. Nevertheless, there
are a number of numerical solvers for one- and two-dimensional problems
\citep[\cfeg][and references therein]{CheKno76, YabAok91, YabIsh91,
SyeTre95, Hoz97, UtsKun98}.

Another possibility is to work with moments of the CBE, in the spirit of
the discussion earlier in this section. The object now is to numerically
solve a truncated set of coupled moments equations, with the caveats that
were given above. Such work has already been done to test stability in
plasmas \citep{Cha95} and extensions to track nonlinear evolution are
under way, both in plasmas and in self-gravitating systems, at Los Alamos
National Laboratory \citep{HabPogXX}. \\

\subsection{Time-Independent (Steady-State) Solutions}
\label{1.subsec.steady}

The aim here is to find time-independent (or steady-state or stationary or
equilibrium) solutions to the CBE, \ie solutions that satisfy $\ptl f/
\ptl t \equiv 0$ in some coordinate system. Eq.~(\ref{1.eq.CBE}) then
becomes
\begin{equation}
  \vv \cdot \frac{\ptl f}{\ptl \xx} -
  \frac{\ptl \Phi}{\ptl \xx} \cdot \frac{\ptl f}{\ptl \pp} = 0,
\label{1.eq.tiCBE}
\end{equation}
where, as before, $\Phi$ is defined self-consistently via {\em Poisson's
equation}:
\begin{equation}
  \Phi(\xx) = -Gm^2 \int \frac{f(\xx',\vv')}{|\xx-\xx'|} \, d\Gamma'
\end{equation}
Despite the superficial similarity between Eqs.~(\ref{1.eq.CBE}) and
(\ref{1.eq.tiCBE}), the process of finding stationary solutions is very
different from that of solving the time-dependent CBE that was discussed
in the previous section. In that case, the task was to compute the
evolution in time, $f(\xx, \vv, t)$, of a DF that obeys the partial
differential equation (\ref{1.eq.CBE}), for an arbitrary initial condition
$f(\xx, \vv, 0)$. The instantaneous form of the DF at time $t$ determines
its form at $t+dt$, self-consistently via the potential.

By contrast, in the stationary problem, the task at hand is to find one or
more time-independent, positive semi-definite functions $f(\xx, \vv)$ that
{\em satisfy} the integro-differential equation (\ref{1.eq.tiCBE}). The
form of the function $f(\xx,\vv)$ will have to be such that it will be
able to support itself self-consistently. In other words, the potential
will have to shuffle phase-space elements in such a way that no change
will be imparted to $f$. It should then come as no surprise that the {\em
existence} of a self-consistent equilibrium corresponding to an arbitrary
potential $\Phi(\xx)$, or density distribution $\rho(\xx)$, is {\em not}
guaranteed. Furthermore, if an equilibrium does exist, it may well {\em
not} be the only one that exists, \ie its {\em uniqueness} is not
guaranteed.

Before proceeding to a brief overview of the techniques and tools
available for the construction of equilibrium models of galaxies, there
are two questions that should be addressed to investigate the legitimacy
of using self-consistent equilibria as realistic approximations of
galaxies.

{\em 1. Are galaxies in a state of equilibrium?} If a galaxy is {\em not}
in a state  of equilibrium, then generally speaking, either (i) it would
undergo a rapid (comparable to a characteristic crossing time) or even
catastrophic evolution, or (ii) it would undergo a slow, secular
evolution, or (iii) it would exhibit some kind of oscillatory behavior.
The first possibility is easily ruled out. If galaxies were evolving
rapidly, one would expect to observe a number of them at different stages
of their evolution. However, with the exception of galaxies in the process
of colliding, merging or having a close encounter with other galaxies, now
or in the near past, most systems seem to have ``regular'' shapes, as
evidenced by the relatively few Hubble types that are needed to classify
most of them. Still, the second and third possibilities can certainly not
be ruled out. Even though neither secular evolution nor oscillatory modes
are directly accessible to observation, there is considerable theoretical
and numerical evidence that they do occur. To name but a few examples,
bars are believed to cause secular evolution in disk galaxies via
redistribution of mass and angular momentum; cooling flows may be slowly
altering the mass distribution near the central regions of elliptical
galaxies; fast galactic flybys and the final stages of galactic mergers
can trigger oscillatory modes that often persist long after the bulk of
the interaction is over; and the presence of one or more companion
galaxies or membership in a dense cluster of galaxies can induce a
permanent quasi-periodic driving. These theoretical and numerical findings
are often corroborated by indirect observational evidence, such as nuclear
galactic starbursts, off-center galactic nuclei, the presence of decoupled
kinematic components inside a galaxy, \etc.

By contrast, the traditional approach to galactic modeling
\citep[\cfeg][p.\ 4 and pp.\ 177-183]{BinTre87} has been to assume that
galaxies are in a state of quasi-equilibrium, and to use adiabatic
invariance to treat the effects of a slowly-varying mean field due to
secular evolution or long-period oscillations. This may be a good
approximation for systems of one degree of freedom, for which adiabatic
invariance was in fact shown, but not necessarily so for systems of more
degrees of freedom, where the adiabatic theorem is weaker and actions may
actually change faster than previously thought \citep{Wei94}. Furthermore,
if the galactic potential is strongly nonintegrable (\cf
\S\ref{1.subsec.steady} under ``Stellar Orbits''), resonant driving of
chaotic orbits can induce changes in the distribution of energies and,
hence, in the bulk distribution of matter, thus causing continuing
evolution to the system \citep{KanAbe95}.

Despite the evidence, very little has been done in terms of constructing
time-dependent self-consistent models that reproduce the visual appearance
of galaxies, though this may not be surprising in view of the difficulties
involved in such a task. However, it can be argued that the study of
stationary solutions to the CBE is still important, even as a first step
towards an understanding of time-dependent systems. Furthermore,
stationary solutions may still be useful approximations of
quasi-stationary galaxies, provided at least that they are {\em
structurally stable}, meaning that they are stable against perturbations
that tend to alter the {\em form} of the potential. Examples of such
perturbations include dynamical friction and noise due to stellar
encounters ({Eq.~\ref{1.eq.langevin}), periodic driving due to companion
galaxies, or an impulse due to a fast galactic flyby. In other words, the
motivation for structural stability analysis is the recognition that most
probably galactic potentials do not have the exact form assigned to them
by galactic dynamicists, and that therefore it is crucial to examine
whether a particular model's stability (and thus its usefulness, at least
as a realistic approximation of a galaxy) strongly depends on small
changes of the functional form of the potential. Again, very little has
been done in terms of investigating the structural stability of
self-consistent galactic models. Most work on this topic terminates with
the construction of a time-independent DF. This dissertation will address
some aspects of this problem (\cf \S\ref{1.sec.mot}).

{\em 2. Does the time-dependent collisionless Boltzmann equation guarantee
convergence towards an equilibrium?} Even if one assumes that galaxies
today are in a state of quasi-equilibrium, they have not always been that
way. They had to form and evolve to their present state. Despite the fact
that the process of galaxy formation is not well understood, it is clear
that after a certain stage in the life of ellipticals, gas dissipation
becomes unimportant and, since then, their evolution is determined by the
CBE. One might therefore attempt to answer the previous question, \ie
whether galaxies are in a state of equilibrium, by investigating whether
the time-dependent CBE dictates an evolution towards a nearly
time-independent final state.

The basic point here is that, because the evolution described by the CBE
is Hamiltonian, the DF cannot reach a state of equilibrium in a pointwise
sense. If $\ptl f/\ptl t$ is nonzero, it will remain nonzero and the
evolution will lead to phase mixing, since the flow is incompressible and
CBE characteristics do not cross. Nevertheless, it is often assumed that
the CBE somehow approaches equilibrium in some appropriate coarse-grained
sense. However, there is no proof that such is the case. Rather, the only
result known to date regarding the asymptotic time behavior of the CBE is
that it admits global existence, \ie given sufficiently smooth initial
conditions one never gets caustics or shocks \citep{Pfa92, Sch91}. One
might still argue that it may just be very hard to prove an approach
towards a coarse-grained equilibrium, but it may nevertheless be
significant that there are exact time-dependent solutions to the CBE,
corresponding to systems that remain bounded in space, which do not
exhibit any approach towards a coarse-grained equilibrium but correspond
to finite-amplitude, undamped oscillations about an otherwise
time-independent equilibrium $f_0$ \citep{LouGer88, Sri89}.

In short, from the preceding discussion it follows that (a) neither
observations nor theoretical considerations rule out --in fact they often
support-- the possibility that at least some galaxies are time-dependent
objects, for example undergoing secular evolution or exhibiting
small-amplitude oscillatory behavior; but that (b) it is still important
to understand stationary systems, both as appropriate idealizations of
some galaxies, and as stepping stones towards the understanding of
nonstationary systems. These comments apply throughout this dissertation,
which concerns mostly the construction of stationary models of elliptical
galaxies.


\underline{\smash{Analytical solutions.}} The main thrust behind the
enterprise of finding analytical solutions to the time-independent CBE is
the {\em Jeans theorem}, which implies that any DF, $f$, that depends on
the phase-space coordinates only via the integrals of motion is a solution
to the CBE. The proof stems from the very definition of an {\em isolating
integral} or {\em global invariant of the motion}, ${\cal I}(\xx,\vv)$, as
being a time-independent conserved quantity
\begin{equation}
  \frac{d\cal{I}}{dt} \equiv
     \frac{d\xx}{dt} \cdot \frac{\ptl\cal{I}}{\ptl\xx} +
     \frac{d\vv}{dt} \cdot \frac{\ptl\cal{I}}{\ptl\vv} =
     \vv             \cdot \frac{\ptl\cal{I}}{\ptl\xx} -
     \frac{\ptl\Phi}{\ptl\xx} \cdot \frac{\ptl\cal{I}}{\ptl\vv} = 0,
\label{1.eq.iom}
\end{equation}
so that any analytical function $f({\cal I}_i)$ of one or more integrals of
the motion ${\cal I}_i$ satisfies the time-independent CBE
(Eq.~\ref{1.eq.tiCBE}):
\begin{equation}
  \vv \cdot \frac{\ptl f({\cal I}_i)}{\ptl \xx} -
  \frac{\ptl \Phi}{\ptl \xx} \cdot \frac{\ptl f({\cal I}_i)}{\ptl \pp} =
  \sum_i \frac{\ptl f({\cal I}_i)}{\ptl {\cal I}_i}
         \left( \vv \cdot \frac{\ptl{\cal I}_i}{\ptl\xx} -
                \frac{\ptl\Phi}{\ptl\xx} \cdot \frac{\ptl{\cal I}_i}{\ptl\vv}
         \right) = 0,
\end{equation}
where the last equality follows from Eq.~(\ref{1.eq.iom}). Therefore, one
can construct stationary models by solving the relatively easier problem
of finding isolating integrals of the motion.

Isolating integrals can be found by means of {\em Noether's theorem}
\citep[\cf][p.\ 88]{Arn89}, which states that for every continuous
symmetry of the potential $\Phi$, there is a globally conserved quantity
(isolating integral of the motion). Thus, for example, the
time-translational symmetry of a stationary or steadily rotating potential
causes the Hamiltonian to be an integral of the motion (identified with
the orbital energy $E = {\scriptstyle \frac{1}{2}}v^2 + \Phi$ in the case
of a system which is stationary with respect to an inertial frame of
reference; or with the Jacobi integral, $E_J$, when  the system is
time-independent in an appropriately chosen rotating frame). If the
potential also possesses an axis of symmetry, the component of the angular
momentum parallel to that axis (say, $L_z$) will also be an integral of
the motion, in addition to the Hamiltonian. In a similar manner, if a
system is spherically symmetric then all three components of the angular
momentum are integrals of the motion.

The construction of some stationary solution (DF) to the CBE would then
entail three steps, namely (1) identifying $n \leq 3$ isolating integrals,
${\cal I}_1, \ldots, {\cal I}_n$, that will reflect the symmetries of the
configuration, (2) writing down the DF as an analytical, positive
semi-definite function of the isolating integrals, $f({\cal I}_1, \ldots,
{\cal I}_n)$, and (3) confirming that the density distribution, $\rho(\xx)
= \int f \, d^3\vv$, in configuration space does indeed possess the
symmetries assumed in step (1).

This last step is necessary for the model to be self-consistent. In
particular, it can be shown that the density distribution $\rho(\xx)$ of a
static (nonrotating) configuration is spherically symmetric if and only if
the DF $f = f(E, L^2)$, \ie it is solely a function of the energy and of
the magnitude of the angular momentum  \citep{PerAly96}. The reason that
the dependence on angular momentum enters via the combination $L^2$, even
though all three components of the angular momentum are conserved, can be
understood considering that $L^2 = r^2 (v_{\theta}^2 + v_{\phi}^2) = r^2
v_T^2$ only depends on the tangential velocity $v_T$, as one would expect
for a spherical system where there is no preference in the $\theta$ or
$\phi$ direction. In the special case where the stellar velocity
distribution is everywhere isotropic, the DF depends solely on the energy,
\ie $f = f(E)$.

One step up in complexity are axisymmetric systems, where two of the three
rotational symmetries that are obeyed by spherical systems cease to exist.
As a consequence, generic time-independent axisymmetric systems have only
two isolating integrals of the motion, namely the energy $E$, and the
component of the angular momentum parallel to the rotation axis $L_z$. If
one relaxes the requirement for axisymmetry, then the only remaining
isolating integral for generic triaxial systems is the energy $E$. The
only known exception is the family of \citet{Sta90} potentials which
possess three integrals of the motion, owing to the fact that their
symmetries are generalizations of a spherical coordinate system in
confocal ellipsoidal coordinates.

\citet{Edd16} showed that there is a unique $f(E)$ that corresponds to an
isotropic spherical mass distribution $\rho(r)$ provided that (i) the
potential $\Phi(r)$ is a monotonic function of $r$, and (ii) $\rho(r)$
drops fast enough with $r$.  However, beyond this simplest of cases, the
task of finding equilibria quickly becomes rather complex and less
fruitful. Although there are ways to construct equilibria of anisotropic
spherical systems as well as axisymmetric systems \citep[\cf][and
references therein]{Dej86, HunQia93}, little is known about the solution
space or the degeneracy of these equilibria. Finally, there is no known
analytical method to construct generic triaxial equilibria (with the
exception of St\"ackel potentials).

Before proceeding to an overview of numerical methods for solving the CBE,
a brief discussion of stellar orbits is in order.


\underline{\smash{Stellar Orbits.}} The orbits of stars moving under the
influence of the gravitational potential $\Phi(\rr)$ generated by the mass
distribution of a galaxy governed by the CBE represent free streaming
along the the characteristics of the CBE. The study of stellar orbits is
complementary to the study of DFs and they both contribute to an
understanding of the evolution dictated by the CBE.

The promise of orbits is that, unlike the enterprise of finding DFs, they
can be calculated for arbitrary potentials, and in fact they serve as the
basis for the construction of numerical solutions to the CBE. Knowledge of
the orbital structures supported by a given potential often allows one to
determine whether the potential can be supported self-consistently, and
orbital stability analysis can provide clues to the types of orbits that
should or should not be included in a self-consistent model and to the
stability of the model.

The downside to this approach is that most orbital work is done within the
context of a fixed ``external'' potential, and it is not always known
whether this potential can be self-consistently reproduced by the mass
distribution of the system. Furthermore, the orbital approach reflects the
behavior of individual orbits and not necessarily of the system as a
whole, so that, for instance, if a family of orbits is shown to be
unstable it does not necessarily mean that the system as whole is also
unstable.

One way of characterizing an orbit is via its set of {\em Lyapunov
characteristic numbers} or {\em Lyapunov exponents}, which determine the
average rate at which two orbits with infinitesimally different initial
conditions deviate with time. The Lyapunov exponents, $\chi_i$, of an
orbit are defined as follows:
\begin{equation}
  \label{1.eq.lyap}
  \chi_i = \lim_{t \to \infty} \, \lim_{\delta Z_i(0) \to 0} \,
         \frac{1}{t} \, \ln \frac{\|\delta Z_i(t) \|}{\|\delta Z_i(0)\|},
\end{equation}
where $\| \delta Z_i(t) \|$ represents some (\eg Euclidean) norm between
the unperturbed and the perturbed orbit at time $t$.

A system with $N$ degrees of freedom lives in a $2N$-dimensional phase
space and thus, there are $2N$ directions along which an orbit can be
perturbed. Therefore, there are $2N$ Lyapunov exponents, $\chi_i$,
associated with every orbit. However, if the system is time-independent
(and therefore energy-conserving), the Lyapunov exponents associated with
perturbations along the direction of motion or perpendicular to the
constant-energy hypersurface have to be zero. It can also be shown that
the remaining $2N-2$ exponents must come in $\pm \chi$ pairs. In other
words, only $N-1$ of the $2N$ exponents can be nonzero and independent.
The largest of the these exponents, also called the {\em maximal Lyapunov
characteristic number} or {\em maximal Lyapunov exponent}, is the one that
usually attracts most practical interest for the reason that it
corresponds to the most unstable direction and dominates the other
Lyapunov exponents. If all Lyapunov exponents associated with an orbit are
zero the orbit is called {\em regular}, otherwise it is called {\em
chaotic}.

There is a close relation between the number of vanishing Lyapunov
exponents and the number of isolating integrals in time-independent
potentials. Much like the case with energy, any perturbation of an orbit
in a direction perpendicular to a ``constant integral'' hypersurface
yields a vanishing Lyapunov exponent. Thus, for example, if a potential
with three degrees of freedom admits three isolating integrals, all six
Lyapunov exponents {\em for all orbits} will be equal to zero (since they
appear in positive/negative pairs) and all orbits will be regular.

The connection between integrals of the motion (or nonvanishing Lyapunov
exponents) and regular orbits can be better seen using the concept of {\em
integrability} of Hamiltonian systems. A Hamiltonian system is called
integrable when the Hamilton-Jacobi equations are completely {\em
separable} in some canonical coordinate system. A necessary and sufficient
condition for separability is for $N$ independent isolating integrals to
exist (independent in the sense that their Poisson bracket $\{I_i,I_j\} =
0$ for all $i,j=1,\ldots,N$). A detailed proof can be found, \eg in
\citet[ \S10]{Arn89}, but, in simple terms, the theorem shows that each
one of the $N$ integrals isolates one degree of freedom by the property
that $\ptl H/\ptl p_i = f(q_i)$.

When the Hamilton-Jacobi equations are separable, the system is integrable
and all orbits are regular, having vanishing Lyapunov exponents. However,
a Hamiltonian need not be integrable to permit the existence of regular
orbits. The phase space of nonintegrable Hamiltonians\footnote{with the
exception of {\em hyperbolic} systems, which contain no regular orbits.}
is densely filled with regular orbits, although they comprise a set of
measure zero. This discontinuous dependence on initial conditions means
that Noether's theorem is not applicable and that these regular orbits are
not constrained by $N$ global isolating integrals. However, they do
respect so-called {\em local integrals}, which are exact invariants of the
motion. In that sense, regular orbits in nonintegrable Hamiltonians are as
legitimate building blocks of time-independent self-consistent models as
their counterparts in integrable Hamiltonians.


\underline{\smash{Numerical solutions.}} Generic triaxial equilibrium
solutions to the CBE can be constructed only using numerical techniques,
which can also be useful for studies of axisymmetric systems. There are
mainly two techniques available today, one due to Schwarzschild
\citep{Sch79} and the other due to Contopoulos and Grosb{\o}l
\citep{ConGro86, ConGro88}. Since numerical techniques for solving the
CBE are central to this dissertation, they are reviewed more extensively
in Chapter~2.


\section{Motivation and Dissertation Overview}
\label{1.sec.mot}

There is considerable theoretical and numerical evidence that if a
Hamiltonian dynamical system has a mass distribution which both is
triaxial and contains a central density cusp then the presence of chaotic
orbits is inevitable. This section presents an overview of why this is so,
after a brief discussion of the observational evidence for triaxiality and
cuspiness in elliptical galaxies, and concludes with an exposition of the
objectives of this dissertation.\\


\subsection{Triaxiality and Central Density Cusps in Elliptical Galaxies}
\label{1.sec.mot.triax}

It is interesting how, as the quality and quantity of observations has
improved over time, the (admittedly weak) consensus on the intrinsic shape
of elliptical galaxies has evolved from axisymmetric to triaxial to
perhaps both axisymmetric and triaxial, depending on the distance from the
galactic center. Some of the main photometric, kinematic, numerical and
theoretical evidence both for and against triaxiality is presented below.

\underline{\smash{Evidence from bulk photometric properties.}}
\citet{Hub26, Hub36} understood that the observed ellipticities of
elliptical galaxies reflect mostly projection effects rather than
intrinsic shapes. However, his dependence solely on photometric
measurements of limited and nonuniform sensitivity prevented him from
making any significant progress, though he attempted an estimate of the
distribution of intrinsic shapes under the assumption that ellipticals
were oblate spheroids randomly oriented in space. A number of other
workers have since tried to deconvolve the three-dimensional shape
distribution as better observational data were becoming available. Most of
the work done with photographic plates used some faint isophote cutoff to
determine ellipticity (and hence Hubble type; see \S\ref{1.sec.prelim}).

More recently, \citet{TreMer95} used modern function estimation techniques
to perform a nonparametric estimate of the frequency function of intrinsic
shapes of a sample of 171 bright ellipticals. The ellipticity for each
galaxy was taken to be the mean ellipticity of the isophotes out to a
specific limiting isophote \citep{Ryd92}. They concluded that the observed
distribution of Hubble types is inconsistent, to a high level of
significance, with both the oblate and prolate hypotheses, due to the
absence of enough round ellipticals (the number of which was overestimated
in older photographic catalogs). By contrast, various distributions of
triaxial intrinsic shapes were consistent with the data, with some
evidence for a broad or bimodal distribution with weak peaks near Hubble
types E1 and E3. In a follow-up paper \citep{TreMer96} they combine these
results with luminosity information to conclude that there is evidence for
two families of elliptical galaxies: fainter ($M_B \gtrsim -20$)
ellipticals tend to be moderately flattened, oblate spheroids, while
brighter ones tend to be more nearly round and triaxial (\citet{KorBen96}
also reached similar conclusions about a dichotomy between triaxial and
spheroidal populations following a different path, but they found that the
two types of ellipticals overlap in brightness; see \S\ref{1.sec.prelim}).

\underline{\smash{Evidence from detailed surface photometry.}}
\citet{Con56} pointed out that, in the absence of any extinction effects,
the projected isophotal curves of an elliptical galaxy whose the
isodensity surfaces are concentric, coaxial and similar ellipsoids, are
concentric and similar ellipses. The projected isophotal ellipses are also
coaxial only if the isodensity surfaces are spheroids (\ie degenerate
ellipsoids with two of their three axes equal) \citep{Fis61}.
Interestingly, only a few years earlier, \citet{Eva51} discovered that the
isophotes of many ellipticals are {\em twisted}, the observational term
for denoting that the projected isophotes are not coaxial. Apparently no
one realized at that time the implication that these observations had for
triaxiality. Although some of the galaxies in Evans's sample later turned
out to be misclassified S0s, isophotal twists have been confirmed a number
of times since then \citep[\cfeg][]{Lil60, Car78, WilSch79} but they were
not linked to triaxiality until after kinematic data became available
(see below).

If twisted isophotes suggest departures from axisymmetry, then the often
observed variation of the isophotal ellipticity with radius
\citep[\cfeg][]{RedShi38, Lil60, Lil66, Car78} as well as the residual
amplitude $a_4$ of the $\cos 4\theta$ term in a Fourier expansion of the
isophotal radius in polar coordinates \citep[\cfeg][]{BenDob88} suggest
departures from ellipsoidal symmetry --- or, more specifically, violation
of at least one of the conditions of concentricity, coaxiality and
similarity of the isodensity ellipsoids.

Nevertheless, more recent observational work seems to cast doubt on at
least some of these arguments in support of triaxiality. For instance, in
a study of a sample of a dozen ellipticals with strong isophotal twists
that cannot be attributed to internal dust absorption, \citet{NieBen92}
argue that a significant fraction of the isophotal twists is actually due
to the two-component nature of those ellipticals, which often bear
S0/SB0-like characteristics, such as boxy isophotes, bars and disks.
Furthermore, \citet{ZepWhi93} warn that many of the observed departures
from triaxiality may be the result of close interactions with other
galaxies, especially in compact groups, rather than a consequence of mass
density being stratified on triaxial ellipsoids.


\underline{\smash{Kinematic evidence.}} It was \citet{Bin78} who spurred
recent interest in the possibility that ellipticals are genuinely triaxial
objects, when he put forth triaxiality as a way of explaining the slow
rotation rate of certain ellipticals, discovered by \citet{BerCap75} and
later confirmed by \citet{Ill77} and others. Specifically, it was found
that many ellipticals rotate slower than required of rotationally
supported oblate spheroids. Even though it would still be possible to save
the oblate spheroidals by attributing the slower net rotation to two
counter-rotating  stellar populations, Binney argued that it would be more
natural to assume that elliptical galaxies are ``hot'' stellar systems
that resist gravitational collapse as a result of the random ``thermal''
motion of their stars (\ie stellar velocity dispersions) rather than
organized rotational motion. If that be the case, there is no reason why
ellipticals would have to be spheroidal; a third integral could hold the
galaxy together in a triaxial configuration.

However, more recent kinematic studies of minor axis rotation have failed
to show that axisymmetry is inconsistent with the data
\citep{FraIll91,NieBen92}, and counter-rotating stellar populations are less
exotic today than they were two decades ago \citep{RubGra92,MerKui94}.

In short, detailed surface photometry observations as well as kinematic
data (i) show clear evidence that many elliptical galaxies are
nonaxisymmetric objects, but (ii) fail to show conclusively that a
sizeable fraction of ellipticals have a mass distribution that is
stratified on genuinely triaxial ellipsoids --- on the contrary, it seems
that most departures from axisymmetry can be attributed to either
environmental effects (especially in the outer regions of the galaxies) or
to the presence of distinct components.

Notwithstanding these observational facts, what matters from a theoretical
perspective is the fact that the axial symmetry is often broken, and
therefore the associated component of the angular momentum no longer
constrains the motion. The important point being that, when a symmetry is
broken, theoretical and numerical work \citep{UdrPfe88,HasNor90,Ath90}
shows that chaos is often introduced. This point is even more valid when
symmetries are broken in a complex manner, as suggested by the
aforementioned observations.


\underline{\smash{Central density cusps.}} An important advancement in
elliptical galaxy research has been the discovery, this decade, that
essentially all elliptical galaxies have central density cusps and/or
harbor central black holes.

More specifically, ground-based \citep{MolSti95} and Hubble Space
Telescope \citep{CraSti93, JafFor94, FerBos94, LauAjh95} observations have
shown that elliptical galaxies essentially never have constant-density
cores, as it was previously thought. Instead, their surface brightness
continues to rise, roughly as a power law, $\Sigma(R) \propto R^{-a}$,
into the smallest observable radius. When surface brightness data are
properly deprojected in three-dimensional space \citep{MerFri95} they
reveal a spatial density cusp $\rho(r) \propto r^{-\gamma}$, with $0
\lesssim \gamma \lesssim 2$. Furthermore, there is mounting evidence
\citep{KorBen96} that the centers of most galaxies harbor massive black
holes (with typical black hole-to-galaxy mass ratios of $10^{-3} \lesssim
M_{bh}/M_{gal} \lesssim 10^{-2}$).

When triaxiality coexists with a central density cusp and/or black hole,
the repercussions on the structure and dynamics of at least the central
regions of the galaxy can be quite profound. Theoretical and numerical
work \citep{GerBin85} indicates that triaxial ellipticals with central
mass concentrations or cusps {\em must} contain a significant number of
chaotic orbits. This is so because resonance overlaps near the center
force at least one family of centrophilic orbits, namely the box orbits,
to jump from one box orbit to another in a near-random fashion.
Furthermore, the contour shape of the time-averaged configuration-space
density of these chaotic box orbits is considerably rounder than the shape
of the galaxy's isodensity contours, and thus they cannot
self-consistently support the underlying triaxial structure. This is not a
problem in axisymmetric systems, where conservation of one component of
the angular momentum prevents orbits from approaching arbitrarily close to
the center.

The situation is now quite different from the one envisaged by
\citet{Sch79, Sch82} when he presented numerical evidence supporting the
existence of triaxial equilibria, thus corroborating Binney's case for
triaxiality. The density profiles of Schwarzschild's models flattened
towards the center and formed a large core. Box orbits, which heavily
populated his models, would not be disrupted by such a soft central force.

In order to make a more detailed investigation of the combined effects of
triaxiality and cuspiness in a realistic model of an elliptical galaxy,
\citet{MerFri96} used Schwarzschild's method to create numerical
equilibria of two model triaxial elliptical galaxies, one with a weak
($\gamma=1$) and one with a strong ($\gamma=2$) cusp. They were only
successful in the weak cusp case, which they accepted as evidence that
strong triaxiality can be inconsistent with a high central density. Hence,
they concluded, ellipticals with strong peaks cannot maintain triaxiality
and will slowly evolve towards axisymmetry, especially in their central
regions.

A possible independent confirmation of this effect comes from $N$-body
simulations suggesting that when a central density cusp develops, either
due to gas accumulation near the center \citep{Udr93,Dub94,BarHer96} or
due to the presence of a massive nuclear black hole
\citep{NorMay85,MerQui98} the system starts evolving towards a more
axisymmetric configuration. The situation is again unlike earlier $N$-body
simulations of gravitational collapse that did not include any nuclear
black hole or dissipative component, which often led to robust
non-axisymmetric end configurations \citep[\cfeg][]{WilJam82, Alb82}.\\


\subsection{Dissertation Overview}

This work has two main objectives. The first is to test Schwarzschild's
method for the construction of numerical self-consistent equilibria, by
using it to create models of Plummer spheres. These are simple integrable
potentials for which analytical DFs, moments and other observables have
been computed and can be compared with numerical results. A question of
particular interest is to determine the suitability of Schwarzschild's
method for the investigation of the nonuniqueness (or degeneracy) of the
DFs, namely the possibility of having alternative DFs with different
velocity distributions but identical mass density distribution. Such
degeneracies are known to exist from analytical work and numerical
techniques can be tested against them. This work is described in Chapter
2.

Once the validity -- and the limitations -- of Schwarzschild's method have
been investigated, the second objective is to use it for the construction
of self-consistent models of the triaxial Dehnen potential, for which no
analytical DFs are known. This study is based on, and complements, a
similar study of this potential by \citet{MerFri96}. The objectives here
are (i) to independently check the robustness of the results of the
previous study, by repeating some of the calculations using slightly
different parameters and techniques, and (ii) to examine whether it is
possible to have alternative DFs that contain significantly different
numbers of chaotic orbits, yet reproduce (at least approximately) the same
mass density distribution.  This work is described in Chapter 3.

Chapter 4 concludes with an overview of the results along with some
suggestions for future work. Some efforts are already underway to test the
stability of these DFs by sampling them to generate ensembles of $N$-body
initial conditions and then evolving these initial conditions into the
future via $N$-body simulations.


==> Chapters/plummer.tex <==
\chapter{SELF-CONSISTENT MODELS OF A PLUMMER SPHERE}

This Chapter concerns the construction of self-consistent Plummer-sphere
equilibria using Schwarzschild's numerical method. After the technique is
presented and discussed, it is used to compute velocity moments and
distributions, which are then compared against analytical results to test
the reliability of the numerical method.


\section{Presentation and Discussion of Schwarzschild's Method}
\label{2.sec.schw}

\citet{Sch79} presented a general numerical method for the construction of
self-consistent DFs, \ie DFs that are solutions to the time-independent
CBE. The technique begins by coarse-graining the mass distribution
$\rho_0(\rr)$ for which a model (a DF) is being sought, using a grid made
of $N_c$ cells, each with mass $m_c^0$ (the existence of such a model is
not {\it a priori} guaranteed). The potential $\Phi_0(\rr)$ corresponding
to $\rho_0(\rr)$ is then derived via Poisson's equation, and a large
number, $N_o$, of orbit templates are computed to create a library of
orbits. Next the contribution of each library orbit to the mass of each
grid cell is calculated. This is easy to do, since the contribution of the
$o$-th orbit, $o=1, \ldots , N_o$, to the mass of the $c$-th grid cell,
$c=1, \ldots , N_c$, is proportional to the number of stars, $w_o \geq 0$,
that populate (or, more accurately, proportional to the weight of) the
orbit, multiplied by the time, $t_c^o$, that the orbit spends in the cell:
$\sum_{o=1}^{N_o} w_o \, t_c^o$. Self-consistency requires finding a set
of $w_o$'s such that
\begin{equation}
\label{2.eq.schw}
q \, \sum_{o=1}^{N_o} w_o \, t_c^o = m_c^0
\quad \mbox{with } w_o \geq 0
\quad \mbox{for all } \, c=1, \ldots , N_c,
\end{equation}
where $q$ is just a normalization factor. This is a typical linear
optimization (or linear programming) problem, which can be solved using a
variety of numerical algorithms (\S\ref{2.sec.optim}).

It is appropriate to precede the application of Schwarzschild's method
with a discussion of potential problems associated with it. Consider the
case of an integrable system where the three integrals of the motion are
$I_1, I_2, I_3$. To every triplet $(I_{1i}, I_{2i}, I_{3i})$ of
permissible values of the integrals correspond one or more orbits (down to
finite square-root-sign and other multiplicities associated with the
symmetries of the Hamiltonian). The (time-averaged) phase-space density of
these orbits
\begin{equation}
  f_{I_{1i}, I_{2i}, I_{3i}}(\xx,\vv) \propto
     \delta_D[I_1(\xx,\vv) - I_{1i}] \, \delta_D[I_2(\xx,\vv) - I_{2i}] \,
     \delta_D[I_3(\xx,\vv) - I_{3i}]
\end{equation}
defines a (time-averaged) configuration-space density
\begin{eqnarray}
\label{2.eq.n}
n_{I_{1i}, I_{2i}, I_{3i}}(\xx) & = & \int\int\int d^3v
                                    f_{I_{1i}, I_{2i}, I_{3i}}(\xx,\vv)
                                    \nonumber \\
                                & = & \int \int \int dI_1 dI_2 dI_3 \,
                                    \frac{\ptl(v_1,v_2,v_3)}{\ptl(I_1,I_2,I_3)}
                                    f_{I_{1i}, I_{2i}, I_{3i}}(\xx,\vv),
\end{eqnarray}
where $\delta_D$ is Dirac's delta. This formulation can be generalized to
the case of a nonintegrable system, where one or two of the integrals of
motion would have to be substituted by the invariant distribution on the
constant-$I_1$ or constant-$\{I_1-I_2\}$ hypersurface \citep{Kan98}.

The construction of a DF that corresponds to a specified mass density
distribution $\rho(\xx)$ is equivalent to finding a weight function
$w(I_1, I_2, I_3)$ such that
\begin{equation}
  \label{2.eq.self}
  \rho(\xx) = \int \int \int dI_1 dI_2 dI_3 \,
              \frac{\ptl(v_1,v_2,v_3)}{\ptl(I_1,I_2,I_3)} \,
              w(I_1, I_2, I_3) \,
              f(\xx, \vv; I_1, I_2, I_3),
\end{equation}
where
\begin{equation}
  f(\xx, \vv; I_1', I_2', I_3') \propto
     \delta_D[I_1(\xx,\vv) - I_1'] \, \delta_D[I_2(\xx,\vv) - I_2'] \,
     \delta_D[I_3(\xx,\vv) - I_3']
\end{equation}
is meant to signify that a continuum of initial conditions in integral
space ${I_1,I_2,I_3}$ is to be considered.

The objective in Schwarzschild's method is to approximate $w(I_1, I_2,
I_3)$ via a set of weights $w_{I_{1i}, I_{2i}, I_{3i}}$ such that the
weighted superposition of $n_{I_{1i}, I_{2i}, I_{3i}}$'s can reproduce the
local density $\rho(\xx)$, or in fact, the mass $m_c$ inside a grid cell
$c$:
\begin{equation}
  m_c \equiv \int_{V_c} d^3x \rho(\xx) =
             \int_{V_c} d^3x \sum_i w_{I_{1i}, I_{2i}, I_{3i}}
                                     n_{{1i}, I_{2i}, I_{3i}}(\xx),
\end{equation}
where $V_c$ is the volume of cell $c$. Note that $n_{I_{1i}, I_{2i},
I_{3i}}(\xx)$ is actually proportional, via the time-average theorem (or
the ergodic theorem, in the case of a chaotic phase space), to the time
$t^o_c$ that orbit $o$ spends inside cell $c$ (Eq.~\ref{2.eq.schw}).

From this formulation, a number of possible conceptual and implementation
problems associated with Schwarzschild's method become apparent and are
outlined below. \\

\subsection{The Ill-Conditioning Problem}
\label{2.sec.ill}

One can see that Eq.~(\ref{2.eq.self}) is the three-dimensional
generalization of an inhomogeneous Fredholm equation of the first kind,
defined via
\begin{equation}
  \label{2.eq.fredholm}
  g(t) = \int_a^b K(t,s)f(s)ds.
\end{equation}
This is a linear integral equation which is  known to often be extremely
ill-conditioned \citep[\cfeg][ \S18 and references therein]{PreTeu92}.
This is so because the kernel $K(t,s)$ generally operates on $f(s)$ as a
smoothing function. When the integral equation is inverted, or in other
words when $f(s)$ is being sought for a given $g(t)$ and for a known
kernel $K(t,s)$, the smoothing operator $K(t,s)$ has to be inverted as
well. The inversion operation can be extremely sensitive to, and amplify,
errors and noise in $g(t)$. This may seem more familiar if one writes the
matrix analog of Eq.~(\ref{2.eq.fredholm}):
\begin{equation}
  \mathbf g = \mathbf K \cdot \mathbf f
\end{equation}
in which case $\mathbf f$ can be found via the matrix inversion operation
\begin{equation}
  \mathbf f = \mathbf K^{-1} \cdot \mathbf g.
\end{equation}
It is well known that this inversion is often ill-conditioned and that the
matrix $\mathbf K$ is not always invertible due to errors and noise. A
successful inversion method will, in general, incorporate some prior
knowledge about the solution, to compensate for the loss of information
due to smoothing.

How does this apply to the problem at hand? Comparison between
Eqs.~(\ref{2.eq.self}) and (\ref{2.eq.fredholm}) shows that the kernel
corresponds to
\begin{equation}
  \label{2.eq.kernel}
  \frac{\ptl(v_1,v_2,v_3)}{\ptl(I_1,I_2,I_3)} \,
  f(\xx, \vv; I_1, I_2, I_3),
\end{equation}
with $\rho(\xx)$ being the known function and $w(I_1, I_2, I_3)$ the
unknown. Even when $\rho(\xx)$ is known precisely (\eg from an analytic
expression), the act of binning configuration space into cells can
introduce errors and noise. Furthermore, Schwarzschild's method has also
been applied to the determination of DFs directly from surface brightness
observations of galaxies, where errors in the measurements are inevitable.
Even worse, however, is the fact that the kernel (\ref{2.eq.kernel}) is
not, in general, known analytically, but has to be evaluated using a
pathological numerical approximation method (\S\ref{2.subsec.kerneval}),
a virtual guarantee for noise amplification.

There have been two kinds of remedies to the ill-conditioned inversion
problem, in the context of Schwarzschild's method. One is to use an
iterative deconvolution scheme, such as the one proposed by \citet{Luc74}
which, however, requires knowledge of a prior, with unknown consequences
to the kind of bias this might have to the solution. This concern is
especially important when one is looking to prove not only the existence
of a solution but also probe its degeneracy. The other remedy most usually
used is to attempt to enforce smoothing, \eg via minimization of the sum
of the squares  of the orbital weights (which minimizes the variations of
the weights from one orbit to the next). This approach is motivated not
only numerically but also physically: stability studies show that
population inversions tend to trigger instabilities \citep{FriPol84,
HolMar85}. \\

\subsection{The Kernel Evaluation}
\label{2.subsec.kerneval}

The kernel itself (Eq.~\ref{2.eq.kernel}) is not known analytically but
has to be approximated. Its evaluation is problematic, because each
orbital template in the library is called upon to represent many other
``nearby'' orbits as well. It is well known, especially for chaotic
orbits, that nearby initial conditions can end up in very different
regions of phase space, making it hard to ensure that the library of
orbits offers a comprehensive coverage of phase space. However, if there
are not enough building blocks available, the model may appear to be
infeasible, even if it actually is not. Furthermore, even if a solution
{\em is} found, there may not be enough of an orbital variety to
effectively explore the degeneracy of the solution space. \\


\subsection{The Error Estimates}

Another source for concern lies in the difficulty of quantifying the error
margins of the numerical DF, \ie the errors of the computed weights. This
means (as in the previous case) that one does not know if lack of
convergence to a solution is a consequence of an inadequate library of
orbital templates or of the non-existence of a solution. However, it also
means that if a solution {\em is} found, one does not know how close to
infeasibility it actually is (a solution too close to infeasibility might
well be infeasible but appear to be feasible within the error margins).
Hence, existence proofs (even within reasonable doubt) are often not
particularly reliable, although a number of workers have pursued them.
Unfortunately no satisfactory solution to this problem has been found yet.
\\


\subsection{Where did the Integrals of the Motion Go?}

Finally, a central problem with Schwarzschild's method is that, at least
in its original formulation, it does not make any connection to the
integrals of the motion, which means that there is no guarantee that the
computed DFs are actually time independent. This problem has been at least
partly addressed in follow-up work, especially by \citep{Van84} for
integrable Hamiltonians, and generalized by \citet{Kan98} for
nonintegrable Hamiltonians as well.

In view of all these complications and concerns, it makes sense to first
apply Schwarzschild's method in detail for the construction of a simple DF
about which many properties are already known analytically and which can
be compared with numerical results, and only then use it for the more
complex triaxial problem. This strategy is pursued in the remainder of
this Chapter, after a brief detour in the following section which
describes an alternative technique for the construction of numerical DFs.


\section{The Contopoulos-Grosb{\o}l Method}

The Contopoulos-Grosb{\o}l method \citep{ConGro86, ConGro88} has been
applied to spiral galaxies, both with \citep{KauCon96} and without a bar,
but not to ellipticals. The method works as follows. First an analytical
form of the galactic potential is obtained by fitting observational data
(typically rotation curves and near-infrared surface photometry) to a
model potential made of a bulge and a disk (axisymmetric component) plus a
spiral perturbation, as well as a bar component (in the case of a barred
spiral). Subsequently, a library of orbits is constructed, comprised of
the ``central'' periodic orbits (which reduce to circular orbits in the
purely axisymmetric case), surrounded by a continuum of trapped orbits
whose radial velocities are dispersed around the central ones in a
Gaussian fashion, presumably induced by diffusion processes. Configuration
space is then coarse-grained with a polar grid, and the contribution of
each orbit to the surface density of each cell is weighted according to
some plausible physical considerations ({\it e.g.}, orbits closer to the
center of the galaxy should be weighted more than those further away,
since the density of the disk drops with distance from the center).
Finally, for each annulus of the grid, a Fast Fourier Transform is
performed with respect to the azimuthal coordinate, which provides the
amplitude and the phase of a few low-order components of the imposed
spiral perturbation. The degree of self-consistency of the model is
determined by comparing the imposed amplitude and phase with the
respective quantities of the response density, obtained from the galactic
potential via Poisson's equation. If the discrepancy exceeds some
tolerance level, the parameters of the model potential and the relative
weights of orbit families are modified manually and the procedure is
repeated.

There are two main differences between the Contopoulos-Grosb{\o}l and the
Schwarzschild method. First, the comparatively loose self-consistency
criterion employed by the former method, as opposed to the latter's
requirement for pointwise agreement between imposed and response density,
makes the point that perhaps the details may not matter too much,
especially in view of the inadequacies of the numerical techniques.
Second, and more important, the former technique makes use of its
inventors' expertise and familiarity with the orbital dynamics of the
systems for which they want to construct self-consistent models. This
allows them to make a judicious choice of the orbits that comprise their
library. As was already mentioned in the discussion of Schwarzschild's
method, and will become more apparent later on, the importance of a
quality library of orbital templates cannot be overemphasized.

In conclusion, there is no reason why the extra physical intuition
encapsulated in the Contopoulos-Grosb{\o}l method cannot be included in a
Schwarzschild type of formulation.


\section{Motivation for Modeling the Plummer Sphere}
\label{2.sec.motiv}

\citet{Plu11} used the potential-density pair that now bears his name to
study the spherical distributions of stars that make up the globular
clusters. Plummer spheres are generally bad approximations of elliptical
galaxies because they deviate from the density profile of ellipticals,
both towards the center and towards infinity (\S\ref{2.sec.dens}).
However, Plummer spheres are simple one-degree-of-freedom (and hence
integrable) systems for which a plethora of analytical results are already
known. Furthermore, DFs for spherical systems are degenerate, in the sense
that there is an infinity of DFs $f(\xx,\vv)$ which, when projected onto
configuration space, correspond to the same mass density distribution
$\rho(r)$.

For these reasons, they serve as a useful testbed for the ability of
numerical techniques (in particular, Schwarzschild's method) to probe (i)
the existence and (ii) the degeneracy of solutions to the CBE, before
these techniques are applied to the more complex problem of constructing
equilibria with three degrees of freedom and studying their degeneracy.
For the latter systems, such as the triaxial Dehnen potential, no
analytical DFs are known, and the presence of chaotic orbits may
exacerbate any preexisting algorithmic problems.

There is yet another motivation for studying a simple system, such as a
Plummer sphere. Although several workers have constructed Schwarzschild
equilibria, few have tested their stability in a thorough manner. An
extension of this project involves sampling of the numerical DFs and
subjecting them to $N$-body simulations to test their stability. However,
the central mass density cusp of the triaxial Dehnen potential poses
several problems to $N$-body algorithms, such as an accelerated rate of
two-body relaxation and the difficulty of profiling a steep cusp with a
limited number of particles. By contrast, Plummer spheres are not cuspy;
they have central cores which tax less the $N$-body algorithms, thus
helping to assure that any observed evolution is genuinely due to
instabilities in the numerical DF.

Interestingly, despite being useful as simple testbeds for Schwarzschild's
technique, Plummer spheres pose unique challenges to the method. In
particular, contrary to orbits in triaxial potentials, which generally
fill volumes in configuration space, all orbits in a spherical system are
planar and represent delta functions in the three-dimensional
configuration space. This  can only make the evaluation of the kernel
(\ref{2.subsec.kerneval}) noisier and the inversion more ill-conditioned,
as will be seen in \S\ref{2.sec.lib}. In that sense, Plummer spheres
represent a ``worst case'' scenario to Schwarzschild's method.

It should be emphasized that this work is not intended to provide an
optimal method for the construction of Plummer DFs. Indeed, for spherical
(and, generally, integrable) systems, it is possible to construct the
matrix $t_c^o$ (time spent by $o$-th orbit in $c$-th cell) without
computing a complete library of orbits \citep[\cf][]{Van84, RicTre84,
Sta87, RixZee97}. However, such alternatives are not an option for
nonintegrable triaxial systems, and therefore will not be considered here.


\section{Density, Potential and Equations of Motion} \label{2.sec.dens}

A Plummer sphere has a mass density distribution defined by the equation
\begin{equation}
  \label{2.eq.plum.rho}
  \rho(r) = \left( \frac{3M}{4\pi b^3} \right)
            \left(1 + \frac{r^2}{b^2} \right) ^ {-5/2},
\end{equation}
where $M$ is the total mass of the sphere and $b$ is a constant that plays
the role of a scale length and determines the degree of central mass
concentration. The asymptotic behavior of the density profile, $\rho(r \to
0) \sim (3M)/(4\pi b^2) = \mbox{const.}$ and $\rho(r \to \infty) \sim
r^{-5}$ means that, unlike realistic elliptical galaxies, a Plummer sphere
has a soft core (instead of a central cusp) and its density falls off too
fast at large radii (the densities of most ellipticals fall off slower
than $r^{-4}$).

The gravitational potential that corresponds to this mass distribution can
be calculated via Poisson's equation:
\begin{equation}
  \nabla^2 \Phi(\xx) = 4 \pi G \rho(\xx)
    \qquad \mbox{or} \qquad
  \Phi(\xx) = -G \, \int\limits_{\Gamma}
  \frac{\rho_0(\xx')}{|\xx-\xx'|} \, d^3 \xx',
\end{equation} 
where $\Gamma$ signifies integration over all configuration space.
When applied to Eq.~(\ref{2.eq.plum.rho}), Poisson's equation yields
\begin{equation}
  \label{2.eq.plum.phi}
  \Phi(r) = - \, \frac{GM}{\sqrt{r^2 + b^2}}.
\end{equation}
The equations of motion for a test particle (star) moving under the
influence of the gravitational field generated by a Plummer sphere can be
computed from Hamilton's equations:
\begin{equation}
  \label{2.eq.plum.acc}
  \ddot{\xx} = - \, \frac{1}{m} \, \frac{\ptl H}{\ptl\xx} =
               - \, GM \, \frac{\xx}{(r^2 + b^2)^{3/2}},
\end{equation}
where $m$ is the mass of the test particle and $H = \frac{1}{2}\pp^2 +
m\Phi(\xx)$ is the Hamiltonian function associated with the particle.

Throughout this work, a system of units will be used for which $G, M,$
and $b$ are all equal to unity. Since
\begin{eqnarray}
  G & = & (6.672 \times 10^{-11}) \, [\mbox{kg}]^{-1} \, [\mbox{m}]^3
                                \, [\mbox{sec}]^{-2} \\
    & = & [10^{11} M_\odot]^{-1} \, [\mbox{kpc}]^3
                                \, [1.491 \times 10^6 \, \mbox{yr}]^{-2},
\end{eqnarray}
this yields a unit of time equal to
\begin{equation}
  1.491 \times 10^6 \, \mbox{yr} \left(\frac{M}{10^{11}M_\odot} \right)^{-1/2}
                                 \left(\frac{b}{1 \mbox{kpc}} \right)^{3/2}.
\end{equation}
The potential-density pair for a Plummer sphere then becomes
\begin{equation}
  \label{2.eq.plum.norm}
  \rho(r) = \frac{3}{4\pi} \left(1 + r^2 \right) ^ {-5/2}
  \qquad \mbox{and} \qquad
  \Phi(r) = - \, \frac{1}{\sqrt{1 + r^2}}.
\end{equation}
\\


\section{Analytical Results}
\label{2.sec.dejon}

The simple form, spherical symmetry and integrability of a Plummer sphere
potential makes it relatively easy to construct analytical DFs $f(E,L^2)$
for these systems. \citet{Dej87} \citep[see also][]{Dej86} worked out, in
considerable detail, DFs for both isotropic and anisotropic Plummer
spheres along with several moments and observable quantities. Dejonghe's
basic trick is to pretend that the density $\rho$ really depends on two
independent quantities, the potential $\Phi$ and a radial coordinate $r$,
thus writing an ``augmented'' mass density distribution $\rho(\Phi,r)$
which, assuming that $\Phi$ is the correct self-consistent potential,
coincides numerically with the true $\rho(r)$. Given this augmented
density, one can then construct mappings between  pairs of functions of
two variables, namely augmented densities $\rho(\Phi,r)$  and
self-consistently related DFs $F(E,L^2)$. Dejonghe focused on a specific
class of augmented densities,
\begin{equation}
  \label{2.eq.rho.augm}
  \rho_q(\Phi,r) = \frac{3}{4\pi} (-\Phi)^{5-q}(1+r^2)^{-q/2},
\end{equation}
with $q \leq 2$ a free parameter. Different choices of $q$ lead to
different DFs with varying degree of anisotropy, all of which yield the
same mass density $\rho(r)$.

\citet{Dej86, Dej87} showed that there is a unique distribution function
$F_q(E,L^2)$ that is consistent with the augmented $\rho_q(\Phi,r)$ of
Eq.~(\ref{2.eq.rho.augm}):
\begin{equation}
  \label{2.eq.DF}
  F_q(E,L^2) =
  \frac{3\Gamma(6-q)}{2(2\pi)^{5/2}\Gamma({\scriptstyle \frac{1}{2}}q)}
             \, (-E)^{7/2-q} {\mathcal H} \left( 0, \frac{1}{2} \: q,
                                          \frac{9}{2}-q, 1; -\frac{L^2}{2E}
                                       \right),
\end{equation}
where $\Gamma(x)$ denotes the gamma function, $E = \frac{1}{2}(v_r^2 +
v_\theta^2 + v_\phi^2) + \Phi(r)$ is the binding energy per unit of mass,
and ${\mathcal H}(a, b, c, d; x)$ can be computed in terms of the
hypergeometric function:
\begin{equation}
  {\mathcal H} (a, b, c, d; x) =
  \left\{
    \begin{array}{l}
      \displaystyle
      \frac{\Gamma(a+b)}{\Gamma(c-a)\Gamma(a+d)} \,
             x^a \, _2F_1(a+b, 1+a-c; a+d; x), \qquad x \leq 1; \\ \\
      \displaystyle
      \frac{\Gamma(a+b)}{\Gamma(d-b)\Gamma(b+c)} \,
             x^{-b} \, _2F_1(a+b, 1+b-d; b+c; \frac{1}{x}), \qquad x \geq 1.
    \end{array}
  \right.
\end{equation}
It can be shown that the following relation exists between $q$ and
Binney's anisotropy parameter $\beta$ \cite[p. 203ff]{BinMam82, BinTre87}:
\begin{equation}
  \beta(r) \equiv 1 - \frac{\sigma_\theta^2}{\sigma_r^2}
           = 1 - \frac{\sigma_\phi^2}{\sigma_r^2}
           = \frac{q}{2} \, \frac{r^2}{1+r^2},
\end{equation}
where $\sigma_r, \sigma_\theta$ and $\sigma_\phi$ are the velocity
dispersions along the corresponding directions, and for a spherically
symmetric system $\sigma_\theta = \sigma_\phi$. From this definition $q$
has the same sign as $\beta$, so that when $q > 0$ the near-radial,
low-angular-momentum orbits prevail, thus creating an excess of radial
dispersion; whereas when $q < 0$ the near-circular, high-angular-momentum
orbits prevail and create an excess of tangential dispersion. When $q =
0$ the system is isotropic.

%%% BEGIN FIGURE

\begin{figure}[p]

\begin{center} 
\epsfig{file=Figures/fig2-1a.eps,width=10.5cm}

\footnotesize{(a)}

\epsfig{file=Figures/fig2-1b.eps,width=10.5cm}

\footnotesize{(b)}
\end{center}


\caption{\label{2.fig.fvt} Distributions of the transverse velocities
normalized so that the escape velocity for given radius equals one. a)
Distributions at radius $r=0$; b) Distributions at radius $r=5$.}

\label{2.fig.1}
\end{figure}

\begin{figure}[t]
\vspace{1cm}
\begin{center}
\epsfig{file=Figures/fig2-2.eps,width=10.5cm}
\end{center}

\caption{\label{2.fig.sigmap} The projected velocity dispersion as a
function of projected radius.}

\label{2.fig.2}
\end{figure}

%%% END FIGURE

The DF~(\ref{2.eq.DF}) contains all the information about the Plummer
sphere it represents, and by integrating it out and computing its various
moments a number of useful quantities and observables can be derived. Two
of them, the distribution of the transverse velocities $F_{v_T}$ and the
projected velocity dispersion $\sigma_p(r_p)$ as a function of the
projected radius $r_p$, are particularly well suited to test
Schwarzschild's method. This is so mainly for two reasons. First, they
reveal velocity information that was not constrained when the
Schwarzschild equilibrium was constructed, thus enabling one to gain a
feeling of the level of irregularity (lack of smoothness) present in the
equilibrium. Second, because $\sigma_p(r_p)$ is an observable that will
also be numerically estimated for the triaxial Dehnen potential, it is
useful to see how robust this estimate is. These two quantities are given
by the following expressions:
\begin{equation}
  \label{2.eq.fvt}
  F_{v_T}(\Phi, r, v_T) = \frac{3}{2^{6-q}\pi} \,
                         \frac{\Gamma(6-q)}{\Gamma({\scriptstyle \frac{1}{2}}q)}
                          \, \frac{L^{9-2q}}{r} \,
                          {\mathcal H} \left( 
                            4-{\scriptstyle \frac{1}{2}}q, q-4, 5-q, 1;
                               -\frac{2\Phi + v_T^2}{L^2} \right)
\end{equation}
and 
\begin{equation}
  \label{2.eq.sprp}
  \sigma_p^2(r_p) = \frac{3\pi}{32} \, \frac{1}{6-q} \,
                    \frac{1}{\sqrt{1+r_p^2}}
                    \left(3 - \frac{5q}{4} \, \frac{r_p^2}{1+r_p^2} \right).
\end{equation}
Figures~\ref{2.fig.1} and \ref{2.fig.2} graphically depict
Eqs.~(\ref{2.eq.fvt}) and (\ref{2.eq.sprp}), respectively, for various
values of $q$. One can infer from Figure~\ref{2.fig.1} that for a
maximally radially anisotropic ($q=2$) system, the mean of the tangential
velocity distribution decreases with increasing distance from the center.
The opposite is true for a tangential ($q < 0$) system, while in the
isotropic ($q=0$) case the shape of the distribution remains unchanged.
This {\em complementarity} property can also be seen in the projected
velocity dispersion, where, at small radii, $\sigma_p^2$ is higher in
radial systems rather than in tangential systems, but the opposite is true
at large radii. Another interesting observation is that all curves
intersect at a single point $\{r_p,\sigma_p^2\} = \{\sqrt{2/3},
3\pi\sqrt{3/5}/64\}$. This is a consequence of the fact that $q$ enters
linearly in both the numerator and denominator of Eq.~(\ref{2.eq.sprp}).

There is an important question one has to address before proceeding to a
meaningful comparison between analytical and numerical predictions. Are
all these analytical results generic or do they reflect the peculiarities
of the decomposition of $\rho(r)$ into an augmented $\rho(\Phi,r)$
(Eq.~\ref{2.eq.rho.augm})? If they do reflect peculiarities of the
decomposition, to what extent would this harm the comparison between
theory and numerical results? Unfortunately, there is no easy answer to
this question. Dejonghe's choice of the functional form for an augmented
density is certainly quite special and serves mathematical convenience
above all. At the same time, there is no general method that would allow
one to explore the entire range of possible augmented densities that
correspond to a given $\rho(r)$. Nevertheless, it may not be unreasonable
to expect that at least certain {\em qualitative} conclusions and trends
might remain valid over a considerable range of choices for the functional
form of the augmented densities. For instance, one might expect that the
complementarity property would transcend specific choices of
$\rho(\Phi,r)$. One might also argue that, given enough templates in the
library of orbits (or, strictly speaking, given an infinity of orbital
templates), Schwarzschild's method ought to be able to select those that
correspond to {\em any} feasible DF, including Dejonghe's. However, even
if it were practical to have an infinity of templates in the library of
orbits, one would also have to force the optimization method to seek a
particular solution, which should somehow be encoded in the cost function
and the constraints of the problem (\S\ref{2.sec.optim}). This is not
always trivial to do, especially if one is limited to, at most, quadratic
cost functions with a linear set of constraints.

The remainder of this Chapter describes the process of computing numerical
DFs of a Plummer sphere using Schwarzschild's method, and then uses these
numerical DFs to extract the distributions of transverse velocities
$F_{v_T}$ and projected velocity dispersions $\sigma_p^2(r_p)$ for
comparison with Dejonghe's corresponding analytical results.




\section{The Library of Orbits} \label{2.sec.lib}

% BEGIN FIGURE

\begin{table}[t]
\begin{center}
\caption{\label{2.tab.ener} Radius ($r$), energy ($E$) and circular
velocity radius ($r_c$) for the 20 equal-mass Plummer sphere shells.}
\begin{tabular}[t]{cccc|cccc}
\hline \hline
Shell & $r$ & $E$ & $r_c$ & Shell & $r$ & $E$ & $r_c$ \\ \hline \hline
 1 & 0.388906 & -0.931999 & 0.271366 & 11 & 1.362183 & -0.591774 & 0.870309 \\
 2 & 0.513324 & -0.889636 & 0.355016 & 12 & 1.487087 & -0.558021 & 0.939376 \\
 3 & 0.613219 & -0.852481 & 0.420643 & 13 & 1.629227 & -0.523110 & 1.016486 \\
 4 & 0.703477 & -0.817894 & 0.478712 & 14 & 1.794980 & -0.486680 & 1.104688 \\
 5 & 0.789792 & -0.784761 & 0.533156 & 15 & 1.994166 & -0.448259 & 1.208643 \\
 6 & 0.875303 & -0.752464 & 0.586069 & 16 & 2.243022 & -0.407193 & 1.336033 \\
 7 & 0.962213 & -0.720590 & 0.638844 & 17 & 2.571058 & -0.362492 & 1.500801 \\
 8 & 1.052389 & -0.688833 & 0.692590 & 18 & 3.039622 & -0.312511 & 1.731995 \\
 9 & 1.147675 & -0.656935 & 0.748334 & 19 & 3.806974 & -0.254057 & 2.104982 \\
10 & 1.250114 & -0.624660 & 0.807155 & 20 & 5.499692 & -0.178895 & 2.921630 \\
\hline \hline
\end{tabular}
\end{center}
\end{table}

% END FIGURE


The first step in the implementation of Schwarzschild's method is the
construction of a library of orbital templates. As explained in
\S\ref{2.sec.schw}, the central concern in this enterprise is to ascertain
that the library offers a comprehensive coverage of the phase space
accessible to the DF that is going to be built. In view of the
inaccuracies introduced in the coarse-graining (\S\ref{2.sec.grid}) and
optimization (\S\ref{2.sec.optim}) stages, it may not matter a lot if
families of orbits that do not support considerable structure in the
sought-after DF are omitted or underrepresented ---the deficit will be
overshadowed by the numerical errors. However, if critical families of
orbits are omitted, the consequence could be that the optimization problem
is infeasible. In such a case, one cannot {\it a priori} know if
infeasibility is due to an inadequate library or because there can exist
no time-independent DF capable of supporting the imposed mass density
distribution $\rho(\xx)$. In practice, these considerations mean that the
next best thing to having an infinite sample of orbital templates would be
to (i) identify the important families of orbits in the potential produced
by $\rho(\xx)$, and (ii) include as many of them as computationally
possible.

The choice of initial conditions for the Plummer sphere is relatively
straightforward. It is an integrable system, and thus all orbits are
regular. All that one has to do is to sample uniformly and as densely as
possible any three independent integrals of the motion (\eg $\{E, L,
L_z\}$). This was implemented as follows. The Plummer sphere was
partitioned into 20 equal-mass, spherical and concentric shells at radii
determined from
\begin{equation}
  m(r) = \int_0^r \rho(r')d^3r' = \frac{Mr^3}{(r^2+b^2)^{3/2}},
\end{equation}
where Eq.~(\ref{2.eq.plum.rho}) was used. At each radius, the value of the
energy on the isopotential surface (which, for spherical systems,
coincides with the isodensity surface) was then computed from
Eq.~(\ref{2.eq.plum.phi}). The radii and energies are shown in
Table \ref{2.tab.ener}.

% BEGIN FIGURE

\begin{figure}[t]

\begin{center}
\epsfig{file=Figures/fig2-3.eps,width=4in}
\end{center}

\caption{The innermost octant of initial conditions for the library of
orbits of a Plummer sphere. The octant was sampled at 40 $(\theta,\phi)$
pairs, selected to be centered on segments of approximately equal area.}

\label{2.fig.ic}
\end{figure}

% END FIGURE

Consequently, the positive octant of each isopotential surface was sampled
at 40 positions, selected to be centered on $(\delta\theta, \delta\phi)$
segments of approximately equal area. This was done by (i) uniformly
sampling the $\theta$-angle variable at 7 values between 0 and $\pi/2$,
(ii) computing the surface area contained within the zones defined by each
consecutive pair of constant-$\theta$ circles via
\begin{equation}
  \label{2.eq.deltaS}
  \delta S(\theta_0,\theta_1) = \int_0^{\pi/2} \int_{\theta_1}^{\theta_2}
              r \sin\theta d\theta d\phi =
              \frac{r\pi}{2} \, \left( \cos\theta_1 - \cos\theta_2 \right),
\end{equation}
(iii) computing the ratio $s$ of the area covered by each zone to the area
$\delta S(0, \frac{1}{7}\frac{\pi}{2})$ covered by the the zone (spherical
triangle) closest to the $z$ axis, and (iv) partitioning each zone in
$[s]$ equal $\delta\phi$ segments. This procedure might have to be
repeated a few times until the fractional part of $s$ would become small
enough so that $[s] \approx s$. The result can be seen in Figure
\ref{2.fig.ic}.

The remaining two integrals were sampled along the line joining the center
of the sphere to every selected point on the octant. The angular momentum
magnitude $L$ was sampled at 5 radial points between the radius of maximum
angular momentum (circular orbit) and the isopotential (zero-velocity)
surface, using
\begin{equation}
  \label{2.eq.L}
  L = L_{\min}' + \frac{4-i}{4} \left( L_{\max}' - L_{\min}' \right),
      \qquad i = 0, \ldots, 4
\end{equation}
where $L_{\min}' = 0.02 \, L_{\max}$ and $L_{\max}' = 0.98 \, L_{\max}$
and $L_{\max} = r_c v_c$ (purely radial or purely circular orbits are not
desirable because they introduce numerical singularities which could be
amplified by the numerical inversion). In order to evaluate $L_{\max}$,
the circular velocity radius $r_c$ and the circular velocity $v_c$ can be
found by combining the expression for centrifugal acceleration
\begin{equation}
  \label{2.eq.centracc}
  \frac{v_c^2}{r_c} = \frac{d\Phi}{dr} = \frac{GMr_c}{(r_c^2+b^2)^{3/2}}
\end{equation}
with conservation of energy at $r=r_c$ (where $v_r=0$)
\begin{equation}
  \frac{1}{2} \, v_c^2 - \frac{GM}{\sqrt{r_c^2+b^2}} = E
\end{equation}
which yields
\begin{equation}
  r_c^2 - 2(r_c^2+b^2) - \frac{2E}{GM} (r_c^2+b^2)^{3/2} = 0.
\end{equation}
This equation can be numerically solved for $r_c$ given the energy $E$ of
the orbit and setting $G=M=b=1$ (see Table \ref{2.tab.ener}). Once $r_c$
is known, $v_c$ can be found from Eq.~(\ref{2.eq.centracc}) and $L_{\max}$
can be evaluated. The initial position then is set to $r_c$, the initial
tangential velocity is $v_t = L/r_c$ and the initial radial velocity is
obtained from the energy.

Finally, the second component of the angular momentum is chosen by
specifying how $v_t$ is decomposed into $v_\theta$ and $v_\phi$,
effectively defining the inclination of the orbital plane with respect to
the $x-y$ plane. A total of 5 angles were computed for every value of $L$
via
\begin{equation}
  \alpha = \frac{i}{5} \cdot \pi, \qquad i=0, \ldots, 4
\end{equation}
so that $v_\phi = v_t \cos\alpha$ and $v_\theta = v_t \sin\alpha$. This
last step could no doubt be avoided. Indeed, all the orbits computed
separately for each value of $\alpha$ will be identical modulo a rotation.
One can take advantage of the spherical symmetry and estimate the
contributions of the entire continuum of orbits in $\alpha \in [0,\pi)$
from an orbit computed for a single $\alpha$. However, such a convenience
is not available in a triaxial potential. Since the purpose of this
experiment is to test Schwarzschild's method with the ultimate goal of
applying it to the triaxial Dehnen potential, no advantage of the
spherical symmetry was taken in the construction of the library of orbits.
In fact, this decision places the Plummer sphere at a disadvantage
compared to a triaxial potential, because, as noted earlier, the Plummer
orbits are delta-functions (planes) in the three-dimensional configuration
space, whereas orbits in triaxial potentials are generally non-planar and,
hopefully, numerically better behaved. In that sense, the Plummer sphere
actually represents a ``worst case'' problem for Schwarzschild's
technique.

At the end of this process, a total of $20 \times 40 \times 5 \times 5 =
20000$ orbital templates are included in the library.

Once the initial conditions of the orbital templates that will make up the
library are selected, the next concern is to ensure that the time-averaged
configuration-space density $n_{I_{1i}, I_{2i}, I_{3i}}(\xx)$ of each
template {\em does} indeed remain (nearly-)time-indepen-dent (\cf
Eq.~\ref{2.eq.n}). This requirement is at least as important as the the
one for comprehensive phase-space coverage. If the building blocks are not
truly time independent, neither will the ``equilibrium'' made out of them
be.

For regular orbits, such as those that populate Plummer spheres, one has
to make sure that each orbit has been given enough time to {\em uniformly}
cover its action torus. If the orbit is closed, or in other words the
ratio of its radial to its azimuthal period is a rational number, then one
would have to integrate that orbit for {\em precisely} an integer number
of the least common multiplier of the two periods. However, regular orbits
of nontrivial potentials are not generally closed, and chaotic orbits are
aperiodic. The time required for uniform coverage of the action torus of
the former, or the constant-$\{I_i\}$ or constant-$\{I_i,I_j\}$
hypersurface of the latter actually depends on the coarse-graining of the
configuration space. Hence it is desirable, for the sake of numerical
convenience, to devise a more general way of figuring out for how long to
integrate an orbit.

\citet{Pfe84} proposed an iterative method, which does not depend on
whether an orbit is regular (closed or open, low- or high-order resonant)
or chaotic. The method consists of the following three steps, in a
slightly different formulation from the original:

\begin{description}

\item[Step 1:] Integrate the orbit over a number $n$ of typical crossing
(or dynamical) times $t_{cr}$ and compute how much time it spends in each
configuration space cell (\S\ref{2.sec.grid}). In other words, compute 
the column $s_{c,1}$ in matrix  $t^o_c$ that corresponds to orbit $o$
integrated over $n$ crossing times. Normalize $s_{c,1}$ so that, \eg
$\displaystyle \sum_c s_{c,1} = 1$.

\item[Step 2:] Integrate orbit $o$ for another $n \, t_{cr}$, thus
obtaining a second column matrix $s_{c,2}$, and normalize again.

\item[Step 3:] If the norm $\| s_{c,1} - s_{c,2} \| > \epsilon$, where
$\epsilon$ is a small positive number of order $10^{-3} \min\{s_{c,1}\}$,
then average $s_{c,1}$ and $s_{c,2}$ and repeat Step 2. Otherwise, the
method has converged and the computation is terminated.

\end{description}
This method is guaranteed to converge (\ie $\displaystyle \lim_{n \to
\infty} s_{c,n}$ exists) for any regular orbit, though it may take several
iterations depending on any high-order resonances and the level of coarse
graining of the grid. Pfenniger found that the method would not always
converge for chaotic orbits, even after long integrations. If, however,
one computes the average of the $s_c$'s that correspond to {\em all} the
chaotic orbits of a given energy, one would usually find much faster
convergence rates \citep{KanMah94} (see also \S\ref{3.sec.optim}).

The \label{2.pag.whynofixedt} importance of using time-independent
building blocks cannot be overemphasized. Some workers have simply
integrated orbits for a ``long enough'' period of time, usually comparable
to a Hubble time $t_H$. The implicit argument here is that if, after more
than a Hubble time, an orbit enters new phase-space domains, that would
have no effect for a real galaxy. However, the orbital integration time is
entirely irrelevant to the age of the universe. These are actually orbital
{\em templates}, in the sense that actual orbits can be sampled anywhere
along them. To give a somewhat contrived example, if nature places a star
near the end of a computed orbit that has been terminated just before it
was about to enter uncharted territory then the model will clearly not be
time-independent.

\begin{figure}[t]
\begin{center}
\epsfig{file=Figures/fig2-5.eps,width=4in}
\end{center}
\caption{\label{2.fig.enercons} Absolute value of relative energy error
after an orbital integration of $\sim 200 \, t_{cr}$}
\end{figure}


The orbits were calculated by integrating the equations of motion
(\ref{2.eq.plum.acc}) using a Bulirsch-Stoer integrator
\citep[ \S7.2.14]{StoBul80} \citep[see also][ \S16.4]{PreTeu92}. This
method was chosen because of its high numerical accuracy and computational
efficiency when integrating smooth functions. However, it later became
apparent that using a symplectic integrator might have been a better
choice, because it would preserve the Hamiltonian nature of the
integration, which would arguably be useful, particularly for the chaotic
orbits of the triaxial Dehnen potential. Moreover, in order to avoid
interpolating between orbital points too far apart, Bulirsch-Stoer was
forced to produce output every tenth of a dynamical time, which was often
too short compared to the method's own choice of integration timestep,
thus losing some efficiency. Nevertheless, Bulirsch-Stoer was twice as
fast as a 5th order Runge-Kutta that was also tried, and it conserved
energy better than one part in $10^8$ for most orbits after 200 dynamical
times (Figure \ref{2.fig.enercons}).


% BEGIN FIGURES

\begin{figure}[p]

\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig2-4-0xy.ps,width=7cm}
\footnotesize{(a)}
\end{center}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig2-4-0xz.ps,width=7cm}
\footnotesize{(b)}
\end{center}
\end{minipage}

\vskip 1cm

\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig2-4-0yz.ps,width=7cm}
\footnotesize{(c)}
\end{center}
\end{minipage}
\hfill
\begin{minipage}{7cm}

\caption{\label{2.fig.orb0} Maximum angular momentum orbit ($L =
L'_{\max}$)}

\end{minipage}

\label{2.fig.4}
\end{figure}


\begin{figure}[p]

\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig2-4-1xy.ps,width=7cm}
\footnotesize{(a)}
\end{center}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig2-4-1xz.ps,width=7cm}
\footnotesize{(b)}
\end{center}
\end{minipage}

\vskip 1cm

\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig2-4-1yz.ps,width=7cm}
\footnotesize{(c)}
\end{center}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\caption{\label{2.fig.orb1} Orbit with angular momentum
         $L = L'_{\min} + \frac{3}{4}(L'_{\max}-L'_{\min})$}
\end{minipage}
\end{figure}


\begin{figure}[p]

\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig2-4-2xy.ps,width=7cm}
\footnotesize{(a)}
\end{center}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig2-4-2xz.ps,width=7cm}
\footnotesize{(b)}
\end{center}
\end{minipage}

\vskip 1cm

\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig2-4-2yz.ps,width=7cm}
\footnotesize{(c)}
\end{center}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\caption{\label{2.fig.orb2} Orbit with angular momentum
         $L = L'_{\min} + \frac{1}{2}(L'_{\max}-L'_{\min})$}
\end{minipage}
\end{figure}


\begin{figure}[p]

\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig2-4-3xy.ps,width=7cm}
\footnotesize{(a)}
\end{center}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig2-4-3xz.ps,width=7cm}
\footnotesize{(b)}
\end{center}
\end{minipage}

\vskip 1cm

\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig2-4-3yz.ps,width=7cm}
\footnotesize{(c)}
\end{center}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\caption{\label{2.fig.orb3} Orbit with angular momentum
         $L = L'_{\min} + \frac{1}{4}(L'_{\max}-L'_{\min})$}
\end{minipage}
\end{figure}


\begin{figure}[p]

\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig2-4-4xy.ps,width=7cm}
\footnotesize{(a)}
\end{center}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig2-4-4xz.ps,width=7cm}
\footnotesize{(b)}
\end{center}
\end{minipage}

\vskip 1cm

\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig2-4-4yz.ps,width=7cm}
\footnotesize{(c)}
\end{center}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\caption{\label{2.fig.orb4} Minimum angular momentum orbit ($L =
L'_{\min}$)}
\end{minipage}
\end{figure}




\begin{figure}[hp]

\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig2-4-10004xy.ps,width=7cm}
\footnotesize{(a)}
\end{center}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig2-4-10004xz.ps,width=7cm}
\footnotesize{(b)}
\end{center}
\end{minipage}

\vskip 1cm

\begin{minipage}{7cm}
\begin{center}
\epsfig{file=Figures/fig2-4-10004yz.ps,width=7cm}
\footnotesize{(c)}
\end{center}
\end{minipage}
\hfill
\begin{minipage}{7cm}
\caption{\label{2.fig.orb10004} Minimum angular momentum orbit ($L =
L'_{\min}$) near the half-mass radius of the Plummer sphere.}
\end{minipage}
\end{figure}

% END FIGURES

Figures \ref{2.fig.orb0} -- \ref{2.fig.orb4} depict the first five orbital
templates in the library. They show the characteristic rosette shapes of
integrable motion. As the angular momentum of each consecutive orbit
decreases, it makes closer passages to the center. At the same time, the
rate of azimuthal motion drops, so that, in 200 circular-orbit dynamical
times, a highly eccentric orbit traces only part of its resonant torus
(Figures \ref{2.fig.orb3} and \ref{2.fig.orb4}). This effect is less
pronounced in the outer parts of the system, where low-angular-momentum
orbits do fill out their resonant tori. However, as can be seen from
Figure \ref{2.fig.orb10004}, there are still considerable density
contrasts between the regions that were covered only once and the regions
the orbit had enough time to visit for a second time. Such differences
exist for near-circular orbits as well (see, for instance, the second and
fourth quadrant of Figure \ref{2.fig.orb2}b) but they are less pronounced
because they are spread over a larger surface area of the torus, owing to
the fact that these orbits' motion in the azimuthal direction is faster.

In spite of what was said earlier regarding integration times, the orbital
templates for the present work were integrated for a fixed period of 200
dynamical times, or more precisely, 200 times the orbital period of a
circular orbit of the same energy. One reason why this was done was to
show how bad the problem of using building blocks that are not truly
time-independent can be in the ``worst-case'' scenario of a Plummer
sphere. More specifically, the results one gets by considering the
computed orbits of low angular momentum as time-independent building
blocks, when in fact they are not, will be compared (\S\ref{2.sec.uni})
with the results one gets by discarding the orbits with the two lowest
values of angular momentum, \ie orbits generated for $i=3$ and $i=4$ in
Eq.~(\ref{2.eq.L}).

However, there was also another, more practical, reason for integrating
over a fixed length of time, namely hardware limitations. An
implementation of Pfenniger's method would require some orbits to be
integrated for very long times. Because the library of orbits is actually
stored on disk (so that velocity moments and other quantities can be
computed once a model is constructed), storing the $20000$ library orbits
would require more disk space than was available for this project.
Furthermore, in the nonintegrable triaxial problem the orbits ``spread
out'' more and the deviation from being truly time-independent building
blocks are less severe. Nevertheless, future work (Chapter 4) will
implement a variation of Pfenniger's method. \\



\section{The Coarse-Graining of Configuration Space}
\label{2.sec.grid}

% BEGIN FIGURE

\begin{figure}[t]
\begin{center}
\epsfig{file=Figures/fig2-grid.eps,width=4in}
\end{center}
\caption{\label{2.fig.grid} The grid used for the coarse-graining of
configuration space}
\end{figure}

% END FIGURE

The configuration space was coarse-grained using a grid similar to the one
used by \citet{MerFri96}, which was in turn based on the grid used by
\citet{Sch79}. The radial dimension is divided by 20 concentric spherical
shells, each containing $1/21$ of the total mass. The last shell extends
to infinity and is not included in the self-consistent problem. These are
the same shells on which the initial conditions were sampled
(\S\ref{2.sec.lib}). Each shell is divided into three segments by the
planes $x=y$, $x=z$ and $y=z$, as shown in Figure \ref{2.fig.grid}, and
each segment is further divided into 16 facets, using a set of three
planes in one direction and three in the vertical direction. For instance,
the lower-left segment is divided by the 3 planes $x/y = 3/2, 5/2$ and
$5$, and similarly by the planes $z/x = 3/2, 5/2$ and $5$. This way, a
total of $20 \times 3 \times 16 = 960$ cells are created. Such a grid
geometry has the numerical advantage that it places similar masses in each
cell.

The time $t^o_c$ (Eq.~\ref{2.eq.schw}) that each orbit spends inside every
cell is computed with high accuracy using the following method. While the
orbit remains in its current cell, time is advanced in steps of $0.1 \,
t_{cr}$ (the library output timestep). When a step of $0.1 \, t_{cr}$
brings the orbit outside its current cell, the timestep is reduced by a
factor of ten, and the process is repeated until the orbit exits the cell
with the smaller timestep, at which point the step is reduced once again
by a factor of ten. This way, $t^o_c$ can be found with an accuracy of
$10^{-3} t_{cr}$. The orbit position between stored library positions is
found using linear interpolation. More sophisticated interpolation
schemes, such as splines, are avoided because they can and do produce
spurious results, especially with irregularly shaped chaotic orbits.

\begin{figure}[hp]
\begin{center}
\epsfig{file=Figures/fig2-6a.eps,width=12cm}

\footnotesize{(a)}

\epsfig{file=Figures/fig2-6b.eps,width=12cm}

\footnotesize{(b)}

\end{center}
\caption{The mass placed by the Plummer density law inside each cell. (a)
All 960 cells. (b) The 48 cells of the lowest energy level.}
\label{2.fig.mc}
\end{figure}


Finally, the mass $m_c$ that the Plummer sphere density law places inside
every cell has to be computed. Given the relatively complex definition of
cell boundaries, the direct analytical evaluation of
\begin{equation}
  m_c = \int_{V_c} \rho(\xx) \, d^3 x
\end{equation}
is somewhat complicated. Instead, the above integral is estimated
numerically by gridding the octant with a very fine rectangular mesh of
variable resolution (finer close to the center, where cells are small, and
becoming coarser with increasing radius) and adding the density
contributions on each grid node. Figure \ref{2.fig.mc} shows mass
variation with cell number. Masses are similar to within a factor of 1.5.


\section{The Optimization Problem}
\label{2.sec.optim}

At the heart of Schwarzschild's method lies the constrained optimization
problem that solves the system of $N_c$ equations [\cf
Eq.~(\ref{2.eq.schw})]
\begin{equation*}
  \sum_{o=1}^{N_o} w_o \, t_c^o = m_c \quad \forall \, o=1, \ldots, N_o
\end{equation*}
subject to
\begin{equation*}
  w_o \geq 0 \quad \forall \, c=1, \ldots, N_c.
\end{equation*}
In general, the problem can be stated as follows:
\begin{eqnarray}
  \label{2.eq.lp1}
  \mbox{Minimize:}   & & f(w_o) \nonumber \\ \nonumber \\
  \mbox{subject to:} & & \sum_{o=1}^{N_o} w_o \, t_c^o = m_c
                         \quad \forall \, c=1, \ldots, N_c\\ \nonumber \\
  \mbox{and:}        & & w_o \geq 0  \quad \forall \, o=1, \ldots, N_o
                         \nonumber
\end{eqnarray}
where $f(w_o)$, the cost or objective function, is a linear function of
the weights. In the astronomical literature, this problem is usually
solved using a SIMPLEX-type algorithm \citep[\cfeg][]{Sch79, RicTre84,
Sta87}, a nonnegative least squares (NNLS) algorithm
\citep[\cfeg][]{Pfe84, Zha96, WozPfe97, RixZee97}, quadratic programming
\citep{MerFri96}, nonlinear optimization \citep{LevSpa94} when the cost
function and/or the constraints are nonlinear, or Lucy's method
\citep{New83, NewBin84, Sta87}. Of these techniques, Lucy's method is
distinctly different, being a Bayesian iterative deconvolution scheme.
\citet{Sta87} used Lucy's method to establish the existence of a solution
and then switched to linear programming to map out the boundaries of the
solution space. \citet{New83} found that linear programming produced DFs
with large short- and long-wavelength fluctuations whereas Lucy's method
produced smooth, rapidly converging DFs.

The present work made use of a quadratic programming (QP) algorithm,
whereby the quadratic part was used solely to impose a level of smoothness
to the distribution of the weights $w_o$. Although Lucy's method was not
implemented or compared against QP, experimentation in the present work
with the QP algorithm (which also includes linear programming (LP) as a
special case) suggests that it is not necessarily intrinsically inferior
to Lucy's algorithm in terms of constructing DFs. QP/LP faithfully does
what it is {\em explicitly} told to do: it precisely obeys the constraints
and optimizes the cost function, and it does that fairly well. However,
once it satisfies its constraints, it does not make any effort to provide
a solution that would be agreeable to the astronomer (such as one that
obeys some smoothness constraint) {\em unless} the astronomer identifies
the extra constraints and demands that they be obeyed (by adding extra
constraints and/or specifying an appropriate cost function).

This may explain some of the frustrating results that certain workers
obtained using LP. By solely requiring that the Plummer density law be
respected in every cell, one tacitly implies that this is all the physics
that there is. But in reality, one also knows that smoothness of the DF
should also be a constraint, both because noisy fluctuations are an
expected numerical artifact of the ill-conditioned inversion, and because
population inversions are known to be sources of instability
(\S\ref{2.sec.ill}). When one enforces some level of smoothness, \eg by
minimizing the sum of the squares of the orbital weights, the solution
does become considerably smoother (though perhaps still not as smooth as a
Lucy solution).

For this work, it was decided that the cleanliness of the constraints
mechanism associated with QP/LP is arguably preferable to the enforced
smoothness of the Lucy algorithm. A maximum likelihood approach could
still be fruitful, but only after all physically motivated constraints
have been exhausted.

Another approach is the NNLS method, which reformulates problem
(\ref{2.eq.lp1}) as follows:
\begin{eqnarray}
  \mbox{Minimize:}   & & \sum_{c=1}^{N_c} \left(
                         m_c - \sum_{o=1}^{N_o} w_o \, t_c^o \right)^2
                         + q f(w_o) \nonumber \\ \\
  \mbox{subject to:} & & w_o \geq 0  \quad \forall \, o=1, \ldots, N_o.
                         \nonumber
\end{eqnarray}
where $q$ is a positive constant. \citet{WozPfe97} argue that an advantage
of NNLS over LP is that, when no exact solution exists, NNLS still
converges to the nearest approximate solution, in a least-squares sense,
whereas LP simply fails (one might argue that such an ``approximate''
solution may actually be quite far away from any physical solution, but it
may still be useful as an indicator of where the problem lies). However,
it is possible to avoid this problem by reformulating the LP problem as
follows:
\begin{eqnarray}
  \label{2.eq.lp2}
  \mbox{Minimize:}   & & f(w_o) + q \sum_{c=1}^{N_c}
                         \left( \lambda_c + \mu_c \right)
                         \nonumber \\ \nonumber \\
  \mbox{subject to:} & & \lambda_c - \mu_c +
                         \sum_{o=1}^{N_o} w_o \, t_c^o = m_c \\ \nonumber \\
  \mbox{and:}        & & w_o, \lambda_c, \mu_c\ \geq 0 
                         \quad \forall \, o=1, \ldots, N_o
                         \quad \mbox{and} \quad \forall \, c=1, \ldots, N_c
                         \nonumber
\end{eqnarray}
where $q$ is a positive constant. This way, the LP algorithm is always
feasible, and any deviations from exact self-consistency can be found by
inspecting the values of $\lambda_c$ and $\mu_c$.

In fact, as was discussed above and will be seen in the next section, if
one simply solves the above LP problem, the solution can be quite noisy
and unphysical, with entire ranges of orbits carrying zero weights. One
can improve upon this undesirable situation by demanding, \eg the
minimization of the sum of the squares of all the orbits, in other words
by solving the problem
\begin{eqnarray}
  \label{2.eq.qp}
  \mbox{Minimize:}   & & f(w_o) + q \sum_{c=1}^{N_c}
                         \left( \lambda_c + \mu_c \right) +
                         p \sum_{o=1}^{N_o} w_o^2 \nonumber \\ \nonumber \\
  \mbox{subject to:} & & \lambda_c - \mu_c +
                         \sum_{o=1}^{N_o} w_o \, t_c^o = m_c \\ \nonumber \\
  \mbox{and:}        & & w_o, \lambda_c, \mu_c\ \geq 0 
                         \quad \forall \, o=1, \ldots, N_o
                         \quad \mbox{and} \quad \forall \, c=1, \ldots, N_c
                         \nonumber
\end{eqnarray}
This has now become a QP problem, defined as
\begin{eqnarray}
  \label{2.eq.qpgen}
  \mbox{Minimize:}   & & c^Tx + \frac{1}{2} x^T Q x \nonumber \\
  \mbox{subject to:} & & Ax = b \\
  \mbox{and:}        & & x \ge 0 \nonumber
\end{eqnarray}
where $A \in R^{m \times n}$, $Q \in R^{n \times n}$ is symmetric positive
semidefinite and $c, x \in R^n, b \in R^m$.

This problem is solved using BPMPD \citep{Mes96b, Mes96a}, a
state-of-the-art implementation of the primal-dual interior point
algorithm for linear and convex quadratic programming problems, kindly
made available by the author. The package includes highly flexible
sparsity handling, fast and robust linear algebra and advanced presolve
techniques. It was compared to several other SIMPLEX and Interior Point
software packages in the public domain and it fared better both in terms
of speed and memory requirements. A $20000 \times 960$ QP problem would
take, depending on the sparsity of the matrix $t^o_c$, between 60 and 150
minutes on a Pentium Pro 200~MHz-class computer with 128 Mb of RAM,
running under Linux.


\section{Nonuniqueness of the Solutions: Comparison with Analytical Results}
\label{2.sec.uni}

The optimization techniques described in the previous section will now be
applied to attempt to reproduce the analytical results presented by
\citet{Dej87}, and in particular Figures \ref{2.fig.1} and \ref{2.fig.2}
(\S\ref{2.sec.dejon}). In order to numerically reproduce the effects of
varying the anisotropy parameter $q$, a series of four optimization runs
was effected, corresponding to a minimization or a maximization of the
number of low angular momentum orbits, performed using LP and QP.

It is appropriate to ask whether a better way exists to numerically
mimic variations of $q$. The answer is most probably yes: it would be
possible to implement additional constraints in every grid cell, that
would enforce a particular anisotropy behavior. However, the aim here
again is to test Schwarzschild's method before it is used to study the
nonuniqueness properties of the triaxial Dehnen potential. Even though one
could attempt to enforce some kind of velocity anisotropy or velocity
dispersion profile to the triaxial case, the lack of knowledge of a DF
carries the danger of demanding a velocity anisotropy or dispersion
profile that is unnatural and hence infeasible. Since the main question
for the triaxial case is whether it is possible to have two DFs with
considerably different amounts of chaos, but both supporting the same mass
distribution, it only makes sense to minimize or maximize the number of
chaotic orbits and see what effect this has to the velocity dispersions.
Therefore, it is appropriate to pose a similar problem in the Plummer case
as well, and attempt to minimize, or maximize, a particular class of
orbits. \\

\subsection{Minimization of Low-$L$ Orbits}

In order to minimize the number of orbits with low angular momenta,
the optimization problem ({\ref{2.eq.lp2}) is solved for the following cost
function:
\begin{equation}
  f(w_o) = \sum_{o=1}^{N_o} \, \lambda(o \!\!\!\! \mod 5) \, w_o,
  \quad \mbox{where} \quad
  \lambda(x) = x - 3 + \left[ \frac{x}{3} \right],
\end{equation}
and the square brackets represent the integer part of the argument. This
formulation makes use of the fact that the orbital templates in the
library come in successive quintets of decreasing angular momentum. The
above definition for $f$ places negative coefficients in front of the two
highest-angular-momentum families of orbits. Since ({\ref{2.eq.lp2}) is a
minimization problem, this causes their weights to be maximized (the more
they are used the lower the cost function becomes). By contrast, the
orbits with the remaining three values of (lower) angular moment have
positive coefficients. Their presence increases the cost function, thus
making them undesirable. 

Figure \ref{2.fig.lminrad} shows the distribution of weights returned by
the optimization software. Figure \ref{2.fig.lminrad}c confirms that the
model is feasible, since the mass placed inside every cell agrees with the
Plummer density law to within single machine precision. It is immediately
apparent from Figure \ref{2.fig.lminrad}a that the LP algorithm uses as
few orbits as it needs to create the model and discards the rest, setting
their weights to essentially zero. There are 4794 orbits with weights
greater than $10^{-10}$, of which only 953 have weights greater than
$10^{-4}$. This number is essentially equal to 960, the number of cells in
the grid. Indeed, linear programming, by construction, finds only as many
nonzeros as the number of constraints (cells).

Obviously, this is an undesirable and unphysical numerical artifact. To
ameliorate the situation, one can solve the QP problem (\ref{2.eq.qp}).
The results are shown in Figure \ref{2.fig.qminrad}. There are now 4492
orbits with $w_o > 10^{-10}$, 4031 of which have $w_o > 10^{-5}$, a
significant improvement. Nevertheless, it is obvious that there is no
reason why more orbits could not be used. Using an alternative quadratic
term and/or increasing the number of cells/constraints could perhaps
involve more orbits in the DF. \\


\subsection{Maximization of Low-$L$ Orbits}

In a way similar to the one used in the previous paragraph, the cost
function is now set to be
\begin{equation}
  f(w_o) = \sum_{o=1}^{N_o} \, \lambda(o \!\!\!\! \mod 5) \, w_o,
  \quad \mbox{where} \quad
  \lambda(x) = 4 - x + \left[ \frac{x}{4} \right],
\end{equation}
The coefficients are now positive for the orbits with the three highest
angular momenta, and negative for the remaining two. The results are shown
in Figure \ref{2.fig.lmaxrad} for the LP problem and in Figure
\ref{2.fig.qmaxrad} for the QP problem. One can see that, even though
self-consistency is satisfied, at least to within the level of
coarse-graining of the model, the DF itself is ``hollow'': the orbits
sampled in the six innermost shells are left almost entirely unpopulated,
both in the LP and the QP models. Such a model seems unphysical and may
quite likely be unstable.

Most probably, this result reflects the problematic low-angular-momentum
orbital templates of the library, which are not truly time-independent. As
was pointed out in \S\ref{2.sec.lib}, low-$L$ orbits close to the center
have entire segments of their resonant tori unoccupied because they were
not integrated for long enough. This effect is less severe with the
low-$L$ orbits in the outer parts of the system, which {\em do} cover
their entire resonant tori albeit not uniformly. The optimization
algorithm then rejects the inner low-$L$ orbits because they violate the
spherical symmetry of the system, though its still manages to use the
outer low-$L$ orbits. However, if the resolution of the grid were to
become finer or the number of constraints otherwise increased, the problem
would most probably become infeasible. \\



\begin{figure}[p]

\vskip -6mm

\begin{center}

\epsfig{file=Figures/fig2-lminrad-w.eps,width=9cm}

\footnotesize{(a)}

\epsfig{file=Figures/fig2-lminrad-wdistr.eps,width=9cm}

\footnotesize{(b)}

\epsfig{file=Figures/fig2-lminrad-res.eps,width=9cm}

\footnotesize{(c)}

\caption{\label{2.fig.lminrad} Minimization of radial orbits -- LP model.
(a) Distribution of weights as a function of orbit number; (b) Frequency
distribution of orbital weights; (c) Relative mass error $\sum_{o=1}^{N_o}
t^o_c w_o/m_c - 1$ as a function of cell number.}

\end{center}
\end{figure}




\begin{figure}[p]

\vskip -6mm

\begin{center}

\epsfig{file=Figures/fig2-qminrad-w.eps,width=9cm}

\footnotesize{(a)}

\epsfig{file=Figures/fig2-qminrad-wdistr.eps,width=9cm}

\footnotesize{(b)}

\epsfig{file=Figures/fig2-qminrad-res.eps,width=9cm}

\footnotesize{(c)}

\caption{\label{2.fig.qminrad} Minimization of radial orbits -- QP model.
(a) Distribution of weights as a function of orbit number; (b) Frequency
distribution of orbital weights; (c) Relative mass error $\sum_{o=1}^{N_o}
t^o_c w_o/m_c - 1$ as a function of cell number.}

\end{center}
\end{figure}




\begin{figure}[p]

\vskip -6mm

\begin{center}

\epsfig{file=Figures/fig2-lmaxrad-w.eps,width=9cm}

\footnotesize{(a)}

\epsfig{file=Figures/fig2-lmaxrad-wdistr.eps,width=9cm}

\footnotesize{(b)}

\epsfig{file=Figures/fig2-lmaxrad-res.eps,width=9cm}

\footnotesize{(c)}

\caption{\label{2.fig.lmaxrad} Maximization of radial orbits -- LP model.
(a) Distribution of weights as a function of orbit number; (b) Frequency
distribution of orbital weights; (c) Relative mass error $\sum_{o=1}^{N_o}
t^o_c w_o/m_c - 1$ as a function of cell number.}

\end{center}
\end{figure}




\begin{figure}[p]

\vskip -6mm

\begin{center}

\epsfig{file=Figures/fig2-qmaxrad-w.eps,width=9cm}

\footnotesize{(a)}

\epsfig{file=Figures/fig2-qmaxrad-wdistr.eps,width=9cm}

\footnotesize{(b)}

\epsfig{file=Figures/fig2-qmaxrad-res.eps,width=9cm}

\footnotesize{(c)}

\caption{\label{2.fig.qmaxrad} Maximization of radial orbits -- QP model.
(a) Distribution of weights as a function of orbit number; (b) Frequency
distribution of orbital weights; (c) Relative mass error $\sum_{o=1}^{N_o}
t^o_c w_o/m_c - 1$ as a function of cell number.}

\end{center}
\end{figure}



\subsection{Transverse Velocity Distributions and Projected Velocity
Dispersions}

The distribution of transverse velocities $ v_T =\sqrt{v_\theta^2 +
v_\phi^2}$ inside a given spherical shell was computed by taking into
account the portions of all orbits entering that shell. To this effect,
the positions and velocities of orbits were sampled at ten times the $0.1
t_{cr}$ library sampling rate, using linear interpolation to avoid
smoothing side-effects of more sophisticated methods such as splines, and
were then converted to spherical coordinates.

The results are shown in Figure \ref{2.fig.lfvt} for the LP DFs and in
Figure \ref{2.fig.qfvt} for the QP DFs. The transverse velocity
distributions constructed from DFs that maximized the number of transverse
orbits (solid lines) clearly follow the trend exhibited by the analytic
models (Figure \ref{2.fig.fvt}, $q=-6$): the mean of their distributions
systematically increases with radius while, at the same time, the area
under the distribution (which is proportional to the local density)
decreases. The numerical distributions appear narrower than the analytic
ones, but this can be explained at least in part from the fact that the
numerical distributions were computed over the range of radii that
corresponds to the width of every shell, whereas the analytical
distributions were found for a single value of the radial coordinate: In
the analytical case, the normalization of the abscissa is such that the
maximum (escape) velocity for that radius is equal to 1. However, for the
numerical distributions, the escape velocity was computed for the {\em
inner} shell radius, where it is faster than for the outer radius, and
hence the shape of the distribution appears more ``compressed'' in the
horizontal direction.

One can also see that the numerical distributions do a rather good job, at
least for small radii, in imitating the bell-like shape of the analytical
distributions. However, it is also obvious that they contain lots of
structure. In particular, there is clear evidence of a bimodal
distribution for most radii, and even hints for a trimodal distribution at
$r=3.04$. It was argued in \S\ref{2.sec.dejon} that Dejonghe's choice of
decomposing $\rho(r)$ is certainly not unique, and so one might be tempted
to interpret the bimodal distributions at face value, as being suggestive
of a DF different from Eq.~(\ref{2.eq.DF}). Nevertheless, such an
interpretation is most probably incorrect. Although the presence of the
bimodal distribution in the numerical DF is beyond doubt, it is most
probably related to the small number of values (5) for which the angular
momentum $L$ was sampled. There were simply not enough orbits with a
continuum of angular momenta to make ``rough edges'' such as these
disappear.

The agreement between analytics and numerics is somewhat worse for the
transverse velocity distributions generated from the numerical DFs that
maximize the number of radial orbits (dashed lines). Here the analytical
results indicate that, as one moves away from the center, the mean of the
velocity distribution should shift to lower values while at the same time
the peak value should grow with respect to the solid-line peak. Indeed, if
one ignores the peak on the lowest-velocity bin, there is a clear trend
that does precisely what the analytical work suggests, modulo bimodal
features and rough edges similar to the ones encountered in the previous
case. However, instead of the distribution being ``absorbed'' smoothly
into the low-velocity bin at large radii, it seemingly disappears quite
abruptly near $r=1.49$. From that point on, there is virtually no
high-transverse-velocity component in the system. In any case, however, it
is not reasonable to expect that this velocity distribution is legitimate,
since the DF itself, which contains hardly any orbits in the low-energy
shells, is unphysical.

Overall, it seems fair to say that the the transverse velocity
distributions, drawn from both numerical DFs, look quite reasonable,
especially in view of the caveats at the beginning of this Chapter.
Furthermore, for those aspects of the distributions that look less
believable, there is usually a readily identifiable numerical reason for
why this is so. Interestingly, there are very few differences between the
velocity distributions computed from the LP and the QP problem.



\begin{figure}[t]
\begin{center}
\epsfig{file=Figures/fig2-lfvta.eps,width=15cm}
\end{center}
\caption{\label{2.fig.lfvt} Distributions of transverse velocities
$F_{v_T}$ at different radii, constructed from DFs obtained from the LP
models. The solid (dashed) line corresponds to the DF that maximizes the
number of transverse (radial) orbits. The abscissae are normalized so that
the maximum (escape) velocity equals to 1.}
\end{figure}

\begin{figure}[t]
\begin{center}
\epsfig{file=Figures/fig2-lfvtb.eps,width=15cm}
\end{center}
\begin{center} Figure 2.17--continued \end{center}
\end{figure}

\begin{figure}[t]
\begin{center}
\epsfig{file=Figures/fig2-lfvtc.eps,width=15cm}
\end{center}
\begin{center} Figure 2.17--continued \end{center}
\end{figure}



\begin{figure}[t]
\begin{center}
\epsfig{file=Figures/fig2-qfvta.eps,width=15cm}
\end{center}
\caption{\label{2.fig.qfvt} Distributions of transverse velocities
$F_{v_T}$ at different radii, constructed from DFs obtained from the QP
models. The solid (dashed) line corresponds to the DF that maximizes the
number of transverse (radial) orbits. The abscissae are normalized so that
the maximum (escape) velocity equals to 1.}
\end{figure}

\begin{figure}[t]
\begin{center}
\epsfig{file=Figures/fig2-qfvtb.eps,width=15cm}
\end{center}
\begin{center} Figure 2.18--continued \end{center}
\end{figure}

\begin{figure}[t]
\begin{center}
\epsfig{file=Figures/fig2-qfvtc.eps,width=15cm}
\end{center}
\begin{center} Figure 2.18--continued \end{center}
\end{figure}


Finally, the projected velocity dispersions were computed on the three
principal planes by projecting the velocities into each plane, dividing
the plane into 20 concentric annuli, and then averaging over the angular
dependence with each annulus. The mean and the variance of the projected
(perpendicular to the principal plane) velocities inside every annulus
were obtained from the usual relations
\begin{equation}
  \langle v_p \rangle = \frac{\sum_i v_{p,i}}{N}
  \quad \mbox{and} \quad
  \langle v_p^2 \rangle = \frac{\sum_i v^2_{p,i}}{N-1},
\end{equation}
where $i$ represents the portions of the projected velocity time series
$v_{p,i} \equiv v_p(t_i)$ of {\em any and all} orbits entering a given
annulus. Again, the positions and velocities of orbits were sampled at ten
times the $0.1 t_{cr}$ library sampling rate, using linear interpolation.
The velocity dispersions were then obtained from
\begin{equation}
  \sigma_p^2 (r_p) = \langle v^2_p \rangle - \langle v_p \rangle ^2
\end{equation}
The results are shown in Figure \ref{2.fig.numsigmap}. The graphs for all
three principal planes look indistinguishable (as a result of the symmetry
of the system but also of the symmetrical way in which the orbits were
selected). Interestingly, the graphs for the DFs derived from LP and QP
also look identical (though upon inspection of the numbers they do differ
at the fraction-of-a-percent level). For these reasons only the plot of
the velocity dispersion obtained from the LP DF on the $x-y$ plane is
shown. Comparison with Figure \ref{2.fig.sigmap} is very good.

\begin{figure}[th]
\begin{center}
\epsfig{file=Figures/fig2-numsigmap,width=15cm}
\end{center}

\caption{\label{2.fig.numsigmap} Projected velocity dispersion as a
function of projected radius. The DF constructed using LP was used to
create this graph, but the graph made from QP is visually identical.}

\end{figure}

